Online Coverage Planning for an Autonomous Weed Mowing Robot with Curvature Constraints

The land used for grazing cattle takes up about one-third of the land in the United States. These areas can be highly rugged. Yet, they need to be maintained to prevent weeds from taking over the nutritious grassland. This can be a daunting task especially in the case of organic farming since herbicides cannot be used. In this paper, we present the design of Cowbot, an autonomous weed mowing robot for pastures. Cowbot is an electric mower designed to operate in the rugged environments on cow pastures and provide a cost-effective method for weed control in organic farms. Path planning for the Cowbot is challenging since weed distribution on pastures is unknown. Given a limited field of view, online path planning is necessary to detect weeds and plan paths to mow them. We study the general online path planning problem for an autonomous mower with curvature and field of view constraints. We develop two online path planning algorithms that are able to utilize new information about weeds to optimize path length and ensure coverage. We deploy our algorithms on the Cowbot and perform field experiments to validate the suitability of our methods for real-time path planning. We also perform extensive simulation experiments which show that our algorithms result in up to 60 % reduction in path length as compared to baseline boustrophedon and random-search based coverage paths.

==> abstract_v0.tex <==
%auto-ignore
\begin{abstract}


   We present the design of our autonomous weed mowing robot for cow pastures called Cowbot.  In organic farming, that also forms the focus group for this work, weed control is challenging and labor intensive since herbicides cannot be used. Cowbot is an electric mower designed to operate in the rugged environments on cow pastures and provide a cost-effective method for weed control in organic farms. It has a finite turning radius and is equipped with a front-mounted weeding implement. The autonomous mower must ensure visual coverage of the pasture to detect weeds and perform path planning to visit and mow them. 
    
    % is challenging and involves planning paths to mow weeds detected online. A coverage path for the mower ensures weeds on the pasture are mowed. However, in the case of localized spatial distribution or low weed density on the pasture, a coverage path results in wastage of resources. 
    
    Since weed distribution on a pasture is not known a priori and is hard to estimate due to environmental factors, online path planning is necessary. We formalize the path planning problem for an autonomous mower with curvature constraints and a finite weed detection range to detect and mow weeds on a pasture. We develop two online path planning algorithms that are able to utilize new information about weeds to optimize path length and ensure coverage. We deploy our algorithms on the Cowbot and perform field experiments to validate the suitability of our methods for real-time path planning. We also perform extensive computational simulations with different weed distributions and show that our algorithms result in upto 60 \% reduction in path length as compared to boustrophedon and random search-based coverage paths.
    
    % The cost of operation is affected by the length of the mower's path on the pasture.
    
    % The length of the mower's path to detect and mow weeds on the pasture is dependent on the density of weeds.
    
    % a pasture significantly affects the path length of the mower and in turn in the. Given a finite weed detection range, it is hard to estimate the weed distribution on a pasture. 
\end{abstract}

==> jump_planner_v0.tex <==
%auto-ignore
\subsection{JUMP Online Planning Algorithm}

% The JUMP planning algorithm performs online planning for an autonomous mower to search and mow weeds in a pasture. It does both detection and mowing simultaneously while executing a boustrophedon like path on the pasture. 

% Consider a rectangular pasture. Without loss of generality, we assume that the longer edge is aligned with the positive x-axis, the shorter edge is aligned with the positive $y$-axis and the bottom left corner of the pasture is placed at $(0,0)$. In the following text, we refer to locations with bigger $y$-coordinate values as being located above locations with smaller $y$-coordinate values, and vice-versa as being located below. Consider a boustrophedon path (parallel to the longer edge) to cover the pasture. Then, the passes in the boustrophedon path are parallel to the $x$-axis and the first pass is along the line $y_p=\mathcal{B}/2$, where $y_p$ is the $y$-coordinate value corresponding to the pass. Let $(x_m,y_m)$ represent the current location of the mower. When the mower detects a new weed, $w_i=(x_i,y_i)$, it adds the weed to its list of weeds, $\mathcal{W}$. When the mower mows a weed, it removes the weed from $\mathcal{W}$. 

%  while executing a boustrophedon like path on the pasture.
% ; and use them to develop the JUMP planning algorithm.

The JUMP algorithm performs online path planning for a mower to simultaneously detect and mow weeds. It introduces the concepts of \emph{jumps} and \emph{spring} within a boustrophedon coverage path and modifies it to optimize path length.
Briefly, \emph{jumps} allow the mower to make detours to mow nearby weeds while traversing a pass, and \emph{spring} behavior allows for variable spacing between consecutive passes on the path resulting in a spring-like stretch and shrink pattern.

Consider the mower's traversal along a pass of the boustrophedon coverage path. Recall that the mower maintains a list $\mathcal{W}$ of weeds detected in the pasture that are yet to be mowed. At each time step along the pass, the mower checks for weeds, $w_i \equiv (x_i,y_i)$, in the weedlist $\mathcal{W}$ that satisfy the following set of constraints:
\begin{align}
\mathcal{C}: ~~&x_i > x_m,& \rm{if}~\theta_p = 0&\nonumber\\
&x_i < x_m,& \rm{if}~\theta_p = \pi&\nonumber\\
&y_i < y_p+\mathcal{S}_w/2&&\nonumber\\
&y_i > y_p+\mathcal{B}/2&&\label{eq:jump_weeds_Wc}
\end{align}
Let $\mathcal{W}_c \subseteq \mathcal{W}$ be the list of weeds that satisfy the constraint set $\mathcal{C}$. The weeds in $\mathcal{W}_c$: 1) lie ahead of the mower in the direction of its motion, 2) lie within the detection field of view of the mower but outside the range of the weeding implement if the mower were to continue straight on the current pass, and 3) lie above the current pass, i.e. $y_i > y_p$. The algorithm then computes a jump $\Delta^k$  (as described in Section \ref{sec:jump}) to each of the weeds $w_k \in \mathcal{W}_c$ from the current pass $(y = y_p)$. Each jump has a start point, $(x_s^k,y_p)$, and an end point, $(x_e^k,y_p)$, that lie on the current pass. The mower makes a search for a jump $\Delta$ with start and end points located at $(x_s,y_p)$ and $(x_e,y_p)$ respectively, that satisfies the following three conditions: 
\begin{enumerate}
    \item start point of the jump coincides with the mower's current location, i.e. $x_{s} = x_m$
    \item end point of the jump is within the detection field of view of the mower, i.e.
    \begin{align*}
    x^k_e < x_m + \mathcal{S}_d, \rm{if}~ \theta_p = 0\\
    x^k_e > x_m - \mathcal{S}_d, \rm{if}~ \theta_p = \pi
    \end{align*}
    % \item end point of the detour is within the \emph{safe} detection field of view of the mower, i.e. $\Delta^k_{end}.x < x_m + \mathcal{S}_d - \frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$, where $\frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$ is the safety margin
    \item there does not exist any weeds $w_i \in \mathcal{W}\setminus\mathcal{W}_c$ on the current pass that are closer than the end point of the jump, i.e. 
    \begin{align*}
    \nexists w_i \in \mathcal{W}\setminus\mathcal{W}_c:
    \begin{cases}
    x^k_{s}<x_i<x^k_{e}, \rm{if}~ \theta_p = 0\\
    x^k_{s}>x_i>x^k_{e}, \rm{if}~ \theta_p = \pi\\
    y_p-\mathcal{B}/2<y_i<y_p+\mathcal{B}/2\end{cases}
    \end{align*}
\end{enumerate}
 
% above the range of the mower's blade in the current pass and 3) lie below the detection field of view limit of the mower on the current pass.
 
A jump that satisfies the three conditions is referred to as feasible. Ties among jumps starting at the same point are broken in favor of the weed with the smallest $y$-coordinate value. If a jump is available at the mower's current location, the mower makes the jump; otherwise it continues moving ahead on the current pass with $\theta_m = \theta_p$. While on a jump, the mower does not check for any new jumps. 

% Note that, such a jump does not lead to any unmowed weeds in $\mathcal{W}$ below ($y_p + \mathcal{B}/2$) at the end of the current pass.


% Also note that, at the start of the pass all weeds in $\mathcal{W}$ lie above ($y_p - \mathcal{B}/2$). In the case of the first pass, it is trivially true by virtue of the pass being at the bottom edge of the pasture.

% Later, we show that this is also true at the start of every pass in the JUMP algorithm. At the end of the first pass, no weeds below ($y_p + \mathcal{B}/2$) are left unmowed.

% At the end of the first pass, JUMP computes the $y_p$ value for the next pass.  is computed as detailed below


% traversing on the next pass in the opposite direction of


% motion.

%  and the set of constraints $\mathcal{C}$ and feasibility conditions for a detour change symmetrically. The detour construction also changes from LSR-RSL to RSL-LSR.
% The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination condition, as detailed below, is met.

At the end of a pass, the planner must compute the $y_p$ value for the next pass. JUMP algorithm does not restrict the spacing between consecutive passes to be constant. The spacing is decided dynamically based on currently available information about weeds in the pasture. This dynamic spacing admits a \emph{spring}-like behavior in the boustrophedon path structure allowing it to stretch or shrink as required. We present two variants of the JUMP algorithm that differ in the maximum permissible separation between consecutive passes, JUMP-HIGH (JH) and JUMP-LOW (JL). The two variants differ only in their computation of $y_p$ value for the next pass. While JUMP-HIGH allows more stretch in the spring when the weed density is low, JUMP-LOW is more conservative and restricts the stretch in the spring to a lower value. JUMP-HIGH computes $y_p(i+1)$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2+\mathcal{B}/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:jumphigh_yp}
\end{align} 
JUMP-LOW computes $y_p(i+1)$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:jumplow_yp}
\end{align}
% \begin{align}
%     % y_p = \rm{minimum}(\min_{\forall i:w_i \in \mathcal{W}}y_i, (y_p+\mathcal{S}_w/2))+\mathcal{B}/2
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_low}
% \end{align}
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_high}
% \end{align}
The $y_p$ computation for the next pass ensures that any weeds in $\mathcal{W}$ left unmowed on the current pass get mowed in future passes. The JUMP planner maintains two invariants through the algorithm execution.
\begin{invariant}
At the start of a pass there does not exist any unmowed weeds in $\mathcal{W}$ below ($y_p-\mathcal{B}/2$). \label{j_inv:pass_start}
\end{invariant}
\begin{proof}
In the case of the first pass, the invariant is trivially true by virtue of the pass being at the bottom edge of the pasture. The computation of $y_p$ ensures that the next pass would ensure the coverage of the bottom most weed in $\mathcal{W}$, thus maintaining the invariant. 
\end{proof}
This brings us to the second invariant of the JUMP algorithm.
\begin{invariant}
Consider $\mathcal{W}_{start}$ to be a snapshot of $\mathcal{W}$ at the start of a pass. At the end of the pass, there does not exist any unmowed weeds in $\mathcal{W}_{start}$ below ($y_p+\mathcal{B}/2$).\label{j_inv:pass_end}
\end{invariant}
\begin{proof}
If the mower traverses the pass without any jumps all weeds in $\mathcal{W}$ below $y_p+\mathcal{B}/2$ are mowed. The JUMP algorithm computes a jump for the mower only in the case there are no weeds on the current pass that will be left unmowed as a result of the jump. This ensures that the invariant is maintained at the end of every pass.
\end{proof}
The two invariants in combination guarantee that the path computed by JUMP algorithm ensures that all detected weeds on the pasture are mowed. 

% By using dynamic spacing to the next pass, the JUMP planner ensures that no unmowed weeds exist in $\mathcal{W}$ below ($y_p - \mathcal{B}/2$) at the start of a new pass at $y_p$.

The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination criteria for JUMP algorithm is met. The termination criteria, evaluated at the end of each pass, is as follows:
\begin{align}
(y_p == B-\mathcal{B}/2) \cap (\mathcal{W} == \phi)\label{eq:jump_terminate}
\end{align}


% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/algos.eps}
% \caption{A pass across the pasture for JUMP and SNAKE algorithms. Gray rectangle represents the robot and red rectangle represents the weeding implement mounted in the front of the robot. Solid disks represent weeds and the black dashed lines show the path taken by the robot when following the respective algorithm. The weeds that get mowed on the path are shown in red, while those left unmowed are shown in blue.}\label{fig:algo_passes}
% \end{figure}


% % \begin{figure}[t]
% % \centering
% % \includegraphics[scale = 0.6]{images/state_transition.eps}
% % \caption{State transition diagram for the local-opt algorithm.}
% % \end{figure}

\begin{algorithm}
\caption{JUMP-planner}\label{algo:jumpAlgo}
\begin{algorithmic}[1]
\Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
\Statex $\mathcal{I}$: vector of 1s
% \Statex
\State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2\Comment{y value corr. to current pass}
\State $\theta_p = 0$\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]\Comment{weed list}
\State mission\_completed = False \Comment{termination flag}
\State jump\_flag = 0 \Comment{0: not on jump, 1: currently on jump}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  initial\_pose \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}
% \State x\_path = path\_f
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [0 : $L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
% \State x\_path = path\_b
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [$L$ : 0, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{not reached end of current\_path}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{jump\_flag == 1}
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{jump is complete}
\State jump\_flag = 0
\EndIf
\State continue
\EndIf
\State $\Delta$ = find\_available\_jump()
\If{$\Delta$ is not empty and $\Delta$ is feasible}
\If{$\theta_p$ == 0}
\State delete steps in current\_path with $x \leq x_e$
\ElsIf{$\theta_p == \pi$}
\State delete steps in current\_path with $x \geq x_e$
\EndIf
\State current\_path.prepend($\Delta$)
\State jump\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{$(y_p == B- \mathcal{B}/2) \cap (\mathcal{W} == \phi)$}
\State mission\_completed = True
\State continue
\EndIf
% \Statex
\State min\_weed\_height = min ($\mathcal{W}.y) + \mathcal{B}$/2
\State $y_p$ = $y_p$ + $\mathcal{S}_w$/2 \Comment (+ $\mathcal{B}$/2) for JUMP-HIGH
\State $y_p$ = min ($y_p$, min\_weed\_height, $B- \mathcal{B}/2$)
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsubsection{Computing the Jump}\label{sec:jump}

In the JUMP planning algorithm, jumps for the autonomous mower to mow nearby weeds are restricted to weeds that lie above the current pass. To construct these jumps, we use primitives from the Dubins' shortest path algorithm for curvature constrained vehicle \cite{dubins}. Specifically we consider Dubins's paths of the type $C^+SC^-$, where $C^+$ and $C^-$ are circular arcs in opposite direction and $S$ is a straight line path. LSR and RSL paths are realizations of the $C^+SC^-$ path type, where R refers to a circular arc in the clockwise direction and L refers to a circular arc in the counter clockwise direction.

We explain the construction of a jump using the geometry shown in Figure \ref{fig:detour_jump}. Given the weed location (\textbf{b}) and $y_p$ value for the current pass, we must compute the start (\textbf{a}) and end (\textbf{c}) points on the pass for the jump. We fix the heading angle at each of the locations to be equal to $\theta_p$. When $\theta_p = 0$, we construct jumps of the type LSR-RSL and when $\theta_p = \pi$, we construct jumps of the type RSL-LSR. In the given example $\theta_p = 0$, hence we show the construction of a LSR-RSL jump. A RSL-LSR jump can be constructed by symmetrically following the same method with $\theta_p = \pi$.

Consider the construction of the shortest LSR path from \textbf{a} $\equiv(x_a,y_a,\theta_a)$ to \textbf{b} $\equiv(x_b,y_b,\theta_b)$. Here, $(x_b,y_b)$ are the location coordinates of the weed, $y_a = y_p$, and $\theta_a=\theta_b=\theta_p$. The only unknown in the two states is $x_a$. We compute the value of $x_a$ such that the L circle at \textbf{a} (shown in red) and the R circle at \textbf{b} (shown in green) are closest to each other but do not intersect at more than one point. The end point of the jump (\textbf{c}) is placed at the same separation on the other side of \textbf{b}, such that $\|x_b-x_a\| = \|x_c-x_b\|$. Then the LSR path from \textbf{a} to \textbf{b} followed by RSL path from \textbf{b} tp \textbf{c} (shown with a solid  black line in the figure), gives the LSR-RSL jump to mow the weed at \textbf{b}.


\begin{figure}[h]
\centering
\includegraphics[scale = 1]{epstopdf images/jump.eps}
\caption{LSR-RSL jump to mow a weed at point \textbf{b}. \textbf{a} and \textbf{c} are the start and end points of the jump on the current pass.}\label{fig:detour_jump}
\end{figure}

% Consider the instantaneous pose ($x_m,y_m,\theta_m$) of an autonomous mower executing a pass on the path planned by the JUMP algorithm. 
%The minimum length path of type LSR occurs when the circles corresponding to the L and R components are closest to each other and do not intersect at more than one-point. %When the separation between the two points is less than $4.\mathcal{R}$ distance, the S component in the shortest LSR (by symmetry in RSL) paths vanishes and the two circles share a common tangent.
 
% The minimum length \textbf{ab} path of type LSR occurs when the tangential circles of L and R components are closest to each other. In our case, if \textbf{b} is less than $4.\mathcal{R}$ above the current pass, the shortest LSR path from \textbf{a} to \textbf{b} will occur when the two circles share a common tangent and the S component vanishes. Given the weed location (\textbf{b}) and $y_p$ value for the current pass we compute the start (\textbf{a}) and end (\textbf{c}) points for the jump such that the two pairs of circles share a common tangent.

% The \textbf{bc} path is constructed similarly with RSL path type. For $\theta_p = \pi$, a symmetrical construction is used to compute RSL-LSR detours.

% To compute minimum length LSR-RSL detour to a weed located above the current pass, we consider the geometry of the detour as shown in Figure \ref{fig:detour_jump}.

%  The positioning and size of the red, green and blue circles in the figure are fixed by the pose vectors at \textbf{a}, \textbf{b} and  \textbf{c}, respectively.









==> jump_planner_v1.tex <==
%auto-ignore
\subsection{JUMP Online Planning Algorithm}

% The JUMP planning algorithm performs online planning for an autonomous mower to search and mow weeds in a pasture. It does both detection and mowing simultaneously while executing a boustrophedon like path on the pasture. 

% Consider a rectangular pasture. Without loss of generality, we assume that the longer edge is aligned with the positive x-axis, the shorter edge is aligned with the positive $y$-axis and the bottom left corner of the pasture is placed at $(0,0)$. In the following text, we refer to locations with bigger $y$-coordinate values as being located above locations with smaller $y$-coordinate values, and vice-versa as being located below. Consider a boustrophedon path (parallel to the longer edge) to cover the pasture. Then, the passes in the boustrophedon path are parallel to the $x$-axis and the first pass is along the line $y_p=\mathcal{B}/2$, where $y_p$ is the $y$-coordinate value corresponding to the pass. Let $(x_m,y_m)$ represent the current location of the mower. When the mower detects a new weed, $w_i=(x_i,y_i)$, it adds the weed to its list of weeds, $\mathcal{W}$. When the mower mows a weed, it removes the weed from $\mathcal{W}$. 

%  while executing a boustrophedon like path on the pasture.
% ; and use them to develop the JUMP planning algorithm.

% The JUMP algorithm performs online path planning for a mower to simultaneously detect and mow weeds. It introduces the concepts of \emph{jumps} and \emph{spring} within a boustrophedon coverage path and modifies it to optimize path length. Briefly, \emph{jumps} allow the mower to make detours to mow nearby weeds while traversing a pass, and \emph{spring} behavior allows for variable spacing between consecutive passes on the path resulting in a spring-like stretch and shrink pattern.

Consider the mower's traversal along a pass of the boustrophedon coverage path. At each time step along the pass, the mower checks for weeds, $w_i \equiv (x_i,y_i)$, in the weedlist $\mathcal{W}$ that satisfy the following criteria:
\begin{align}
\mathcal{C}: ~~&x_i > x_m,& \rm{if}~\theta_p = 0&\nonumber\\
&x_i < x_m,& \rm{if}~\theta_p = \pi&\nonumber\\
&y_i < y_p+\mathcal{S}_w/2&&\nonumber\\
&y_i > y_p+\mathcal{B}/2&&\label{eq:jump_weeds_Wc}
\end{align}
Let $\mathcal{W}_c \subseteq \mathcal{W}$ be the list of weeds that satisfy the constraint set $\mathcal{C}$. The planner then computes a jump (detour) $\Delta^k$  (as described in Section \ref{sec:jump}) to each of the weeds $w_k \in \mathcal{W}_c$ from the current pass $(y = y_p)$. Each jump has a start point, $(x_s^k,y_p)$, and an end point, $(x_e^k,y_p)$, that lie on the current pass. The planner makes a search for a jump that satisfies the following three conditions:
\begin{enumerate}
    \item start point of the jump coincides with the mower's current location, i.e. $x_{s}^k = x_m$
    \item end point of the jump is within the FOV, i.e.
    \begin{align*}
    x^k_e < x_m + \mathcal{S}_d, \rm{if}~ \theta_p = 0\\
    x^k_e > x_m - \mathcal{S}_d, \rm{if}~ \theta_p = \pi
    \end{align*}
    % \item end point of the detour is within the \emph{safe} detection field of view of the mower, i.e. $\Delta^k_{end}.x < x_m + \mathcal{S}_d - \frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$, where $\frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$ is the safety margin
    \item the jump does not lead to any missed weeds:
    \begin{align*}
    \nexists w_i \in \mathcal{W}\setminus\mathcal{W}_c:
    \begin{cases}
    x^k_{s}<x_i<x^k_{e}, \rm{if}~ \theta_p = 0\\
    x^k_{s}>x_i>x^k_{e}, \rm{if}~ \theta_p = \pi\\
    y_p-\mathcal{B}/2<y_i<y_p+\mathcal{B}/2\end{cases}
    \end{align*}
\end{enumerate}
 
% above the range of the mower's blade in the current pass and 3) lie below the detection field of view limit of the mower on the current pass.
 
A jump that satisfies the three conditions is referred to as feasible. Ties among jumps are broken in favor of weeds with the smaller $y$-coordinate. If a feasible jump is available at the mower's current location, the mower makes the jump; otherwise it continues moving ahead on the current pass. While on a jump, the mower does not check for new jumps. 

% Note that, such a jump does not lead to any unmowed weeds in $\mathcal{W}$ below ($y_p + \mathcal{B}/2$) at the end of the current pass.


% Also note that, at the start of the pass all weeds in $\mathcal{W}$ lie above ($y_p - \mathcal{B}/2$). In the case of the first pass, it is trivially true by virtue of the pass being at the bottom edge of the pasture.

% Later, we show that this is also true at the start of every pass in the JUMP algorithm. At the end of the first pass, no weeds below ($y_p + \mathcal{B}/2$) are left unmowed.

% At the end of the first pass, JUMP computes the $y_p$ value for the next pass.  is computed as detailed below


% traversing on the next pass in the opposite direction of


% motion.

%  and the set of constraints $\mathcal{C}$ and feasibility conditions for a detour change symmetrically. The detour construction also changes from LSR-RSL to RSL-LSR.
% The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination condition, as detailed below, is met.

At the end of a pass, the planner must compute the $y_p$ value for the next pass with $\theta_p = \pi - \theta_p$. JUMP algorithm does not restrict the spacing between consecutive passes to be constant. This dynamic spacing admits a \emph{spring}-like behavior in the boustrophedon path structure allowing it to stretch or shrink as required. We present two variants of the JUMP algorithm, JUMP-HIGH (JH) and JUMP-LOW (JL), that differ in their computation of $y_p$ value for the next pass. JUMP-HIGH computes $y_p(i+1)$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2+\mathcal{B}/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:jumphigh_yp}
\end{align} 
JUMP-LOW computes $y_p(i+1)$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:jumplow_yp}
\end{align}
The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination criteria for JUMP algorithm is met. The termination criteria, evaluated at the end of each pass, is as follows:
\begin{align}
(y_p == B-\mathcal{B}/2) \cap (\mathcal{W} == \phi)\label{eq:jump_terminate}
\end{align}
% \begin{align}
%     % y_p = \rm{minimum}(\min_{\forall i:w_i \in \mathcal{W}}y_i, (y_p+\mathcal{S}_w/2))+\mathcal{B}/2
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_low}
% \end{align}
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_high}
% \end{align}
% The $y_p$ computation for the next pass ensures that any weeds in $\mathcal{W}$ left unmowed on the current pass get mowed in future passes. 
The JUMP planner (Algorithm \ref{algo:jumpAlgo}) maintains two invariants at each step through the execution of the path.
\begin{invariant}
At the start of a pass there does not exist any unmowed weeds in $\mathcal{W}$ below ($y_p-\mathcal{B}/2$). \label{j_inv:pass_start}
\end{invariant}
\begin{proof}
In the case of the first pass, the invariant is trivially true by virtue of the pass being at the bottom edge of the pasture. The computation of $y_p$ ensures that the next pass would ensure the coverage of the bottom most weed in $\mathcal{W}$, thus maintaining the invariant. 
\end{proof}
% This brings us to the second invariant of the JUMP algorithm.
\begin{invariant}
Consider $\mathcal{W}_{start}$ to be a snapshot of $\mathcal{W}$ at the start of a pass. At the end of the pass, there does not exist any unmowed weeds in $\mathcal{W}_{start}$ below ($y_p+\mathcal{B}/2$).\label{j_inv:pass_end}
\end{invariant}
\begin{proof}
If the mower traverses the pass without any jumps all weeds in $\mathcal{W}$ below $y_p+\mathcal{B}/2$ are mowed. The JUMP algorithm computes a jump for the mower only in the case there are no weeds in $\mathcal{W}$ on the current pass that will be left unmowed as a result of the jump. This ensures that the invariant is maintained at the end of every pass.
\end{proof}
The two invariants in combination guarantee that the path computed by JUMP algorithm ensures that all detected weeds on the pasture are mowed. 

% By using dynamic spacing to the next pass, the JUMP planner ensures that no unmowed weeds exist in $\mathcal{W}$ below ($y_p - \mathcal{B}/2$) at the start of a new pass at $y_p$.



% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/algos.eps}
% \caption{A pass across the pasture for JUMP and SNAKE algorithms. Gray rectangle represents the robot and red rectangle represents the weeding implement mounted in the front of the robot. Solid disks represent weeds and the black dashed lines show the path taken by the robot when following the respective algorithm. The weeds that get mowed on the path are shown in red, while those left unmowed are shown in blue.}\label{fig:algo_passes}
% \end{figure}


% % \begin{figure}[t]
% % \centering
% % \includegraphics[scale = 0.6]{images/state_transition.eps}
% % \caption{State transition diagram for the local-opt algorithm.}
% % \end{figure}

\begin{algorithm}
\caption{JUMP-planner ($L,B,\mathcal{S}_d,\mathcal{S}_w,\mathcal{B},\mathcal{R}$)}\label{algo:jumpAlgo}
\begin{algorithmic}[1]
% \Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
% \Statex $\mathcal{I}$: vector of 1s
% \Statex
% \State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2%\Comment{y value corr. to current pass}
\State $\theta_p = 0$%\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]%\Comment{weed list}
\State mission\_completed = False %\Comment{termination flag}
\State jump\_flag = 0 %\Comment{0: not on jump, 1: currently on jump}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  \{$0,~\mathcal{B}$/2, 0\}% \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}\Comment{$\mathcal{I}$: vector of 1s}
% \State x\_path = path\_f
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [0 : $L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$] 
\ElsIf{$\theta_p == \pi$}
% \State x\_path = path\_b
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [$L$ : 0, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{not reached end of current\_path}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{jump\_flag == 1}
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{jump is complete}
\State jump\_flag = 0
\EndIf
\State continue
\EndIf
\State $\Delta$ = find\_available\_jump()
\If{$\Delta$ is not empty and $\Delta$ is feasible}
\If{$\theta_p$ == 0}
\State delete steps in current\_path with $x \leq x_e$
\ElsIf{$\theta_p == \pi$}
\State delete steps in current\_path with $x \geq x_e$
\EndIf
\State current\_path.prepend($\Delta$)
\State jump\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{$(y_p == B- \mathcal{B}/2) \cap (\mathcal{W} == \phi)$}
\State mission\_completed = True
\State \Return
\EndIf
% \Statex
\State min\_weed\_height = min ($\mathcal{W}.y) + \mathcal{B}$/2
\State $y_p$ = $y_p$ + $\mathcal{S}_w$/2 \Comment (+ $\mathcal{B}$/2) for JUMP-HIGH
\State $y_p$ = min ($y_p$, min\_weed\_height, $B- \mathcal{B}/2$)
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsubsection{Computing the Jump}\label{sec:jump}
Jumps for the mower to mow nearby weeds are restricted to weeds that lie above the current pass. To construct these jumps, we use primitives from the Dubins' shortest path algorithm for curvature constrained vehicle \cite{dubins}. Specifically we consider Dubins's paths of the type $C^+SC^-$, where $C^+$ and $C^-$ are circular arcs in opposite direction and $S$ is a straight line path. LSR and RSL paths are realizations of the $C^+SC^-$ path type, where R refers to a circular arc in the clockwise direction and L refers to a circular arc in the counter clockwise direction.

We explain the construction of a jump using the geometry shown in Figure \ref{fig:detour_jump}. Given the weed location (\textbf{b}) and $y_p$ value for the current pass, we must compute the start (\textbf{a}) and end (\textbf{c}) points on the pass for the jump. We fix the heading angle at each of the locations to be equal to $\theta_p$. When $\theta_p = 0$, we construct jumps of the type LSR-RSL and when $\theta_p = \pi$, we construct jumps of the type RSL-LSR. In the given example $\theta_p = 0$, hence we show the construction of a LSR-RSL jump. A RSL-LSR jump can be constructed by symmetrically following the same method with $\theta_p = \pi$.

Consider the construction of the shortest LSR path from \textbf{a} $\equiv(x_a,y_a,\theta_a)$ to \textbf{b} $\equiv(x_b,y_b,\theta_b)$. Here, $(x_b,y_b)$ are the location coordinates of the weed, $y_a = y_p$, and $\theta_a=\theta_b=\theta_p$. The only unknown in the two states is $x_a$. We compute the value of $x_a$ such that the L circle at \textbf{a} (shown in red) and the R circle at \textbf{b} (shown in green) are closest to each other but do not intersect at more than one point. The end point of the jump (\textbf{c}) is placed at the same separation on the other side of \textbf{b}, such that $\|x_b-x_a\| = \|x_c-x_b\|$. Then the LSR path from \textbf{a} to \textbf{b} followed by RSL path from \textbf{b} tp \textbf{c} (shown with a solid  black line in the figure), gives the LSR-RSL jump to mow the weed at \textbf{b}.


\begin{figure}[h]
\centering
\includegraphics[scale = 1]{images/jump.eps}
\caption{LSR-RSL jump to mow a weed at point \textbf{b}. \textbf{a} and \textbf{c} are the start and end points of the jump on the current pass.}\label{fig:detour_jump}
\end{figure}

% Consider the instantaneous pose ($x_m,y_m,\theta_m$) of an autonomous mower executing a pass on the path planned by the JUMP algorithm. 
%The minimum length path of type LSR occurs when the circles corresponding to the L and R components are closest to each other and do not intersect at more than one-point. %When the separation between the two points is less than $4.\mathcal{R}$ distance, the S component in the shortest LSR (by symmetry in RSL) paths vanishes and the two circles share a common tangent.
 
% The minimum length \textbf{ab} path of type LSR occurs when the tangential circles of L and R components are closest to each other. In our case, if \textbf{b} is less than $4.\mathcal{R}$ above the current pass, the shortest LSR path from \textbf{a} to \textbf{b} will occur when the two circles share a common tangent and the S component vanishes. Given the weed location (\textbf{b}) and $y_p$ value for the current pass we compute the start (\textbf{a}) and end (\textbf{c}) points for the jump such that the two pairs of circles share a common tangent.

% The \textbf{bc} path is constructed similarly with RSL path type. For $\theta_p = \pi$, a symmetrical construction is used to compute RSL-LSR detours.

% To compute minimum length LSR-RSL detour to a weed located above the current pass, we consider the geometry of the detour as shown in Figure \ref{fig:detour_jump}.

%  The positioning and size of the red, green and blue circles in the figure are fixed by the pose vectors at \textbf{a}, \textbf{b} and  \textbf{c}, respectively.









==> jump_planner_v2.tex <==
%auto-ignore
\subsection{JUMP Online Planning Algorithm}

% The JUMP planning algorithm performs online planning for an autonomous mower to search and mow weeds in a pasture. It does both detection and mowing simultaneously while executing a boustrophedon like path on the pasture. 

% Consider a rectangular pasture. Without loss of generality, we assume that the longer edge is aligned with the positive x-axis, the shorter edge is aligned with the positive $y$-axis and the bottom left corner of the pasture is placed at $(0,0)$. In the following text, we refer to locations with bigger $y$-coordinate values as being located above locations with smaller $y$-coordinate values, and vice-versa as being located below. Consider a boustrophedon path (parallel to the longer edge) to cover the pasture. Then, the passes in the boustrophedon path are parallel to the $x$-axis and the first pass is along the line $y_p=\mathcal{B}/2$, where $y_p$ is the $y$-coordinate value corresponding to the pass. Let $(x_m,y_m)$ represent the current location of the mower. When the mower detects a new weed, $w_i=(x_i,y_i)$, it adds the weed to its list of weeds, $\mathcal{W}$. When the mower mows a weed, it removes the weed from $\mathcal{W}$. 

%  while executing a boustrophedon like path on the pasture.
% ; and use them to develop the JUMP planning algorithm.

The JUMP planner (Algorithm \ref{algo:jumpAlgo}) modifies a boustrophedon coverage path by introducing the concepts of \emph{jumps} and \emph{spring}. Briefly, \emph{jumps} allow the mower to make detours to mow nearby weeds while traversing a pass and \emph{spring} refers to variable spacing between consecutive passes on the path resulting in a stretch and shrink pattern. To explain the working of the planner, we consider the mower's traversal along a pass of the boustrophedon coverage path. At each time step along the pass, the mower checks for weeds, $w_i \equiv (x_i,y_i)$, in the weedlist $\mathcal{W}$ that satisfy the following criteria:
\begin{align}
\mathcal{C}: ~~&x_i > x_m,& \rm{if}~\theta_p = 0&\nonumber\\
&x_i < x_m,& \rm{if}~\theta_p = \pi&\nonumber\\
&y_i < y_p+\mathcal{S}_w/2&&\nonumber\\
&y_i > y_p+\mathcal{B}/2&&\label{eq:jump_weeds_Wc}
\end{align}
Let $\mathcal{W}_c \subseteq \mathcal{W}$ be the list of weeds that satisfy the constraint set $\mathcal{C}$. The planner then computes a jump (detour) $\Delta^k$, as explained in Section \ref{sec:jump}, to each of the weeds $w_k \in \mathcal{W}_c$ from the current pass $(y = y_p)$. Each jump has a start point, $(x_s^k,y_p)$, and an end point, $(x_e^k,y_p)$, that lie on the current pass. The planner makes a search for jumps that satisfy the following criteria:
\begin{enumerate}
    \item starts at mower's current location, i.e. $x_{s}^k = x_m$
    % \item start point of the jump coincides with the mower's current location, i.e. $x_{s}^k = x_m$
    \item end point of the jump is within the FOV, i.e.
    \begin{align*}
    x^k_e < x_m + \mathcal{S}_d, \rm{if}~ \theta_p = 0\\
    x^k_e > x_m - \mathcal{S}_d, \rm{if}~ \theta_p = \pi
    \end{align*}
    % \item end point of the detour is within the \emph{safe} detection field of view of the mower, i.e. $\Delta^k_{end}.x < x_m + \mathcal{S}_d - \frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$, where $\frac{\mathcal{S}_d\mathcal{B}}{\mathcal{S}_w}$ is the safety margin
    \item the jump does not lead to any missed weeds:
    \begin{align*}
    \nexists w_i \in \mathcal{W}\setminus\mathcal{W}_c:
    \begin{cases}
    x^k_{s}<x_i<x^k_{e}, \rm{if}~ \theta_p = 0\\
    x^k_{s}>x_i>x^k_{e}, \rm{if}~ \theta_p = \pi\\
    y_p-\mathcal{B}/2<y_i<y_p+\mathcal{B}/2\end{cases}
    \end{align*}
\end{enumerate}
 
% above the range of the mower's blade in the current pass and 3) lie below the detection field of view limit of the mower on the current pass.
 
A jump that satisfies the three conditions is referred to as feasible. Ties among jumps are broken in favor of weeds with the smaller $y$-coordinate. If a feasible jump is available at the mower's current location, the mower makes the jump; otherwise it continues moving ahead on the current pass. While on a jump, the mower does not check for new jumps. 

% Note that, such a jump does not lead to any unmowed weeds in $\mathcal{W}$ below ($y_p + \mathcal{B}/2$) at the end of the current pass.


% Also note that, at the start of the pass all weeds in $\mathcal{W}$ lie above ($y_p - \mathcal{B}/2$). In the case of the first pass, it is trivially true by virtue of the pass being at the bottom edge of the pasture.

% Later, we show that this is also true at the start of every pass in the JUMP algorithm. At the end of the first pass, no weeds below ($y_p + \mathcal{B}/2$) are left unmowed.

% At the end of the first pass, JUMP computes the $y_p$ value for the next pass.  is computed as detailed below


% traversing on the next pass in the opposite direction of


% motion.

%  and the set of constraints $\mathcal{C}$ and feasibility conditions for a detour change symmetrically. The detour construction also changes from LSR-RSL to RSL-LSR.
% The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination condition, as detailed below, is met.

At the end of a pass, the planner must compute the $y_p$ value for the next pass with $\theta_p = \pi - \theta_p$. JUMP algorithm does not restrict the spacing between consecutive passes to be constant. This dynamic spacing admits a \emph{spring}-like behavior in the boustrophedon path structure allowing it to stretch or shrink as required. % We present two variants of the JUMP algorithm, JUMP-HIGH (JH) and JUMP-LOW (JL), that differ in their computation of $y_p$ value for the next pass. JUMP-HIGH computes $y_p(i+1)$ as follows:
$y_p(i+1)$ is computed as follows:
% \begin{align}
%     y_p(i+1) = \rm{min}
%     \begin{cases}
%     \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
%     y_p(i)+\mathcal{S}_w/2+\mathcal{B}/2\\
%     B-\mathcal{B}/2
%     \end{cases}\label{eq:jumphigh_yp}
% \end{align} 
% JUMP-LOW computes $y_p(i+1)$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    \min\limits_{\forall i:w_i \in \mathcal{W}} y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:jumplow_yp}
\end{align}
The mower continues traversing on consecutive passes across the pasture, alternating its direction of motion, until the termination criteria for JUMP algorithm is met. The termination criteria, evaluated at the end of each pass, is as follows:
\begin{align}
(y_p == B-\mathcal{B}/2) \cap (\mathcal{W} == \phi)\label{eq:jump_terminate}
\end{align}
% \begin{align}
%     % y_p = \rm{minimum}(\min_{\forall i:w_i \in \mathcal{W}}y_i, (y_p+\mathcal{S}_w/2))+\mathcal{B}/2
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_low}
% \end{align}
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2),B-\mathcal{B}/2)\label{eq:yp_compute_jump_high}
% \end{align}
% The $y_p$ computation for the next pass ensures that any weeds in $\mathcal{W}$ left unmowed on the current pass get mowed in future passes. 
The JUMP planner maintains two invariants at each step through the execution of the path.
\begin{invariant}
At the start of a pass there does not exist any unmowed weeds in $\mathcal{W}$ below ($y_p-\mathcal{B}/2$). \label{j_inv:pass_start}
\end{invariant}
\begin{proof}
The invariant is true on the first pass by virtue of it being at the bottom edge of the pasture. In consecutive passes, the computation of $y_p$ ensures coverage of the bottom most weed in $\mathcal{W}$, thus maintaining the invariant. 
\end{proof}
% This brings us to the second invariant of the JUMP algorithm.
\begin{invariant}
Consider $\mathcal{W}_{start}$ to be a snapshot of $\mathcal{W}$ at the start of a pass. At the end of the pass, there does not exist any unmowed weeds in $\mathcal{W}_{start}$ below ($y_p+\mathcal{B}/2$).\label{j_inv:pass_end}
\end{invariant}
\begin{proof}
If the mower traverses a pass without any jumps, all weeds in $\mathcal{W}$ below $y_p+\mathcal{B}/2$ are mowed. The planner computes a jump for the mower only in the case when there are no weeds in $\mathcal{W}$ on the current pass that will be skipped as a result of the jump. This ensures that the invariant is maintained at the end of every pass.
\end{proof}
The two invariants in combination guarantee that the path computed by JUMP algorithm ensures that all detected weeds on the pasture are mowed. 

% By using dynamic spacing to the next pass, the JUMP planner ensures that no unmowed weeds exist in $\mathcal{W}$ below ($y_p - \mathcal{B}/2$) at the start of a new pass at $y_p$.



% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/algos.eps}
% \caption{A pass across the pasture for JUMP and SNAKE algorithms. Gray rectangle represents the robot and red rectangle represents the weeding implement mounted in the front of the robot. Solid disks represent weeds and the black dashed lines show the path taken by the robot when following the respective algorithm. The weeds that get mowed on the path are shown in red, while those left unmowed are shown in blue.}\label{fig:algo_passes}
% \end{figure}


% % \begin{figure}[t]
% % \centering
% % \includegraphics[scale = 0.6]{images/state_transition.eps}
% % \caption{State transition diagram for the local-opt algorithm.}
% % \end{figure}

\begin{algorithm}
\caption{JUMP-planner ($L,B,\mathcal{S}_d,\mathcal{S}_w,\mathcal{B},\mathcal{R}$)}\label{algo:jumpAlgo}
\begin{algorithmic}[1]
% \Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
% \Statex $\mathcal{I}$: vector of 1s
% \Statex
% \State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2%\Comment{y value corr. to current pass}
\State $\theta_p = 0$%\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]%\Comment{weed list}
\State mission\_completed = False %\Comment{termination flag}
\State jump\_flag = 0 %\Comment{0: not on jump, 1: currently on jump}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  \{$0,~\mathcal{B}$/2, 0\}% \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}\Comment{$\mathcal{I}$: vector of 1s}
% \State x\_path = path\_f
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [0 : $L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$] 
\ElsIf{$\theta_p == \pi$}
% \State x\_path = path\_b
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State current\_path = [$L$ : 0, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
% \State current\_path = [x\_path, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{not reached end of current\_path}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{jump\_flag == 1}
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{jump is complete}
\State jump\_flag = 0
\EndIf
\State continue
\EndIf
\State $\Delta$ = find\_available\_jump()
\If{$\Delta$ is not empty and $\Delta$ is feasible}
\If{$\theta_p$ == 0}
\State delete steps in current\_path with $x \leq x_e$
\ElsIf{$\theta_p == \pi$}
\State delete steps in current\_path with $x \geq x_e$
\EndIf
\State current\_path.prepend($\Delta$)
\State jump\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{$(y_p == B- \mathcal{B}/2) \cap (\mathcal{W} == \phi)$}
\State mission\_completed = True
\State \Return
\EndIf
% \Statex
\State min\_weed\_height = min ($\mathcal{W}.y) + \mathcal{B}$/2
\State $y_p$ = $y_p$ + $\mathcal{S}_w$/2
\State $y_p$ = min ($y_p$, min\_weed\_height, $B- \mathcal{B}/2$)
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsubsection{Computing the Jump}\label{sec:jump} 
Jumps are detours for the mower to mow nearby weeds that lie above the current pass. Each jump comprises of two sub-paths: first, to go \emph{up} to the weed location from the current pass and second, to come back \emph{down} to the current pass. Hence, the start and end points of a jump are located on the current pass. We use Dubins' paths of type RSL and LSR to construct sub-paths for a jump. If $\theta_p = 0$, the first sub-path is a LSR path to go to the weed location and the second sub-path is a RSL path to come back to the current pass. If $\theta_p = \pi$, the first sub-path is of type RSL and the second sub-path is of type LSR. Figure \ref{fig:detour_jump} shows a LSR-RSL jump construction for the mower with $\theta_p = 0$. Here, \textbf{a} and \textbf{c} are the start and end points of the jump such that $(x_b-x_a) = (x_c-x_b)$.



% Jumps for the mower to mow nearby weeds are restricted to weeds that lie above the current pass. To construct these jumps, we use primitives from the Dubins' shortest path algorithm for curvature constrained vehicle \cite{dubins}. Specifically we consider Dubins's paths of the type $C^+SC^-$, where $C^+$ and $C^-$ are circular arcs in opposite direction and $S$ is a straight line path. LSR and RSL paths are realizations of the $C^+SC^-$ path type, where R refers to a circular arc in the clockwise direction and L refers to a circular arc in the counter clockwise direction.

% Consider the jump construction shown in Figure \ref{fig:detour_jump} to mow a weed located at \textbf{b}. Heading angle for the mower at the start $(x_a,y_a)$, middle $(x_b,y_b)$ and end $(x_c,y_c)$ points of the jump is set to $\theta_p$. Since $\theta_p=0$ in the example, we construct a LSR path from \textbf{a} to \textbf{b} and a RSL path from \textbf{b} to \textbf{c}. The start point is placed on the current pass such that the L circle at \textbf{a} (shown in red) and the R circle at \textbf{b} (shown in green) are closest to each other but do not intersect at more than one point. The end point of the jump, \textbf{c}, is placed such that $(x_b-x_a) = (x_c-x_b)$. The LSR-RSL path from \textbf{a} to \textbf{c} passing through \textbf{b} forms the jump for the mower to mow the weed located at \textbf{b}.

% Given a weed location (\textbf{b}) and $y_p$ value for the current pass, we must compute t

% %  We refer to the jump shown in Figure \ref{fig:detour_jump}.
%  We fix the heading angle at each of the locations to be equal to $\theta_p$. When $\theta_p = 0$, we construct jumps of the type LSR-RSL and when $\theta_p = \pi$, we construct jumps of the type RSL-LSR. In the given example $\theta_p = 0$, hence we show the construction of a LSR-RSL jump. A RSL-LSR jump can be constructed by symmetrically following the same method with $\theta_p = \pi$.

% Consider the construction of the shortest LSR path from \textbf{a} $\equiv(x_a,y_a,\theta_a)$ to \textbf{b} $\equiv(x_b,y_b,\theta_b)$. Here, $(x_b,y_b)$ mark the weed location, $y_a = y_p$, and $\theta_a=\theta_b=\theta_p$. The only unknown in the two states is $x_a$. We compute the value of $x_a$ such that the L circle at \textbf{a} (shown in red) and the R circle at \textbf{b} (shown in green) are closest to each other but do not intersect at more than one point. The end point of the jump (\textbf{c}) is placed at the same separation on the other side of \textbf{b}, such that $\|x_b-x_a\| = \|x_c-x_b\|$. Then the LSR path from \textbf{a} to \textbf{b} followed by RSL path from \textbf{b} tp \textbf{c} (shown with a solid  black line in the figure), gives the LSR-RSL jump to mow the weed at \textbf{b}.


\begin{figure}[h]
\centering
\includegraphics[scale = .8]{epstopdf images/jump.eps}
\caption{LSR-RSL jump to mow a weed at point \textbf{b}. \textbf{a} and \textbf{c} are the start and end points of the jump on the current pass.}\label{fig:detour_jump}
\end{figure}

% Consider the instantaneous pose ($x_m,y_m,\theta_m$) of an autonomous mower executing a pass on the path planned by the JUMP algorithm. 
%The minimum length path of type LSR occurs when the circles corresponding to the L and R components are closest to each other and do not intersect at more than one-point. %When the separation between the two points is less than $4.\mathcal{R}$ distance, the S component in the shortest LSR (by symmetry in RSL) paths vanishes and the two circles share a common tangent.
 
% The minimum length \textbf{ab} path of type LSR occurs when the tangential circles of L and R components are closest to each other. In our case, if \textbf{b} is less than $4.\mathcal{R}$ above the current pass, the shortest LSR path from \textbf{a} to \textbf{b} will occur when the two circles share a common tangent and the S component vanishes. Given the weed location (\textbf{b}) and $y_p$ value for the current pass we compute the start (\textbf{a}) and end (\textbf{c}) points for the jump such that the two pairs of circles share a common tangent.

% The \textbf{bc} path is constructed similarly with RSL path type. For $\theta_p = \pi$, a symmetrical construction is used to compute RSL-LSR detours.

% To compute minimum length LSR-RSL detour to a weed located above the current pass, we consider the geometry of the detour as shown in Figure \ref{fig:detour_jump}.

%  The positioning and size of the red, green and blue circles in the figure are fixed by the pose vectors at \textbf{a}, \textbf{b} and  \textbf{c}, respectively.









==> kinematic_model.tex <==
%auto-ignore
\section{Kinematic Model}

In this section we develop a geometric model for Cowbot's kinematics. Cowbot is built on a four-wheeled rear steered platform with traction on the front two wheels. To design a navigation controller for the Cowbot, we need to model its kinematics. In previous work, Rajamani \cite{rajamani} designed a geometric model for vehicles with independent steering control on both front and rear wheels, and described its extension to front steered vehicles. Since a rear steered vehicle turns opposite to the steering angle direction, there are important differences from Rajamani's vehicle model. We extend their model to rear steered front wheel drivetrain vehicles and derive the associated kinematic equations. We use a bicycle model to represent the four wheeled robot (similar to \cite{wangQI} and \cite{rajamani}) where the front two wheels and the rear two wheels are each represented by a single wheel at the front and rear of the bicycle model, respectively. The robot is assumed to operate in the two dimensional plane with zero slip at either of the two wheels. The zero slip assumption is standard in the literature \cite{rajamani} and holds true at low speeds. 

% Existing vehicle models in the literature \cite{rajeshRajamani} describe the geometry of front steered vehicle models. However, there does not exist any work in the literature that describes the kinematics of a rear steered vehicle. 

Consider the top view of the bicycle model shown in Figure \ref{fig:rsteer_front_ref}. The front wheel of the model is centered at $\mathcal F$ and the rear wheel is centered at $\mathcal{B}$. Wheel base of the bicycle model is of length L. The robot moves with a speed $v$ with heading angle $\theta$ about the positive x-axis. The velocity at each of the wheels is in the direction of motion of the wheels and is shown in the figure with dashed arrows. Steering angle of the rear wheel, $\delta$, is measured with respect to the longitudinal axis of the robot model. Both, heading and steering angles of the model are measured in the counter clockwise direction. As shown in the figure, the robot turns in the direction opposite to the steering angle of the rear wheel. This is because the instantaneous center of rotation (ICR), found as the intersection of the rotation axes of the front and rear wheels, is located on the opposite side at $\mathcal{I}$ resulting in an angular velocity in the direction opposite to the rear wheel steering angle.

We consider a 3-tuple state for the bicycle model, $<x,y,\theta>$. Here $(x,y)$ are the location coordinates of a fixed reference point on the model and $\theta$ is the heading direction of the bicycle. The inputs to the model are the magnitude of the velocity, $v$, and the steering angle of the rear wheel, $\delta$. The choice of reference point may be driven by the application. For instance, in the case when a sensor or actuator is mounted in the front of the robot, the center of the front wheel of the bicycle would be an obvious choice for the reference point. Other applications might require the rear end or another point on the robot to be tracked as the reference point. In the following, we consider three reference point locations on the model and derive the kinematic equations for the bicycle model at each of these points.

\subsection{Reference point at the front wheel}

Consider the bicycle model geometry in Figure \ref{fig:rsteer_front_ref} that shows the reference point location at the center of the front wheel. Let the coordinates of the reference point be $\mathcal F \equiv (x_f,y_f)$. On the robot, this point corresponds to the center of the front axle. To derive the state gradient equations, we consider $\triangle \mathcal{FIB}$. The turn radius R at the reference point $\mathcal F$ may then be calculate as follows:
\begin{flalign}
\tan{\delta} = \frac{\rm{L}}{\rm{R}} ~~ \Rightarrow ~~ \rm{R} = \frac{\rm{L}}{\tan{\delta}}\label{eq:fref_R}
\end{flalign}
\noindent Using equation (\ref{eq:fref_R}), we compute the state gradient equations as follows:
\begin{flalign}
&\dot x = v\cos{\theta}\\
&\dot y = v\sin{\theta}\\
&\dot \theta  = -\omega = -\frac{v}{\rm{R}} = -\frac{v}{\rm{L}}\tan{\delta}
\end{flalign}

\begin{figure}
    \centering
    \includegraphics[width=0.75\columnwidth,clip]{images/rsteer_front_ref_newsymb.png}
    \caption{Bicycle model for a rear steered vehicle with front wheel drivetrain. The figure shows the steering geometry when the reference point is located at the center of the front wheel ($\mathcal F$).}\label{fig:rsteer_front_ref}
\end{figure}


% \subsection{Reference point at the rear wheel}
% Consider the bicycle model geometry in Figure \ref{fig:rsteer_rear_ref} that shows the reference point location at the center of the rear wheel. Let the coordinates of the reference point be $\mathcal B \equiv (x_b,y_b)$. On the robot, this point corresponds to the center of the rear axle. To derive the state gradient equations, we consider $\triangle \mathcal{FIB}$. The turn radius R at the reference point $\mathcal B$ may then be calculate as follows.
% \begin{flalign}
% \sin{\delta} = \frac{\rm{L}}{\rm{R}} ~~ \Rightarrow ~~ \rm{R} = \frac{\rm{L}}{\sin{\delta}}\label{eq:rref_R}
% \end{flalign}
% \noindent Using equation (\ref{eq:rref_R}), we find the state gradient equations as follows.
% \begin{flalign}
% &\dot x = v\cos{(\theta+\delta)}\\
% &\dot y = v\sin{(\theta+\delta)}\\
% &\dot \theta  = -\omega = -\frac{v}{\rm{R}} = -\frac{v}{\rm{L}}\sin{\delta}
% \end{flalign}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\columnwidth,clip]{images/rsteer_rear_ref_newsymb.png}
%     \caption{Bicycle model for a rear steered vehicle with front wheel drivetrain. The figure shows the steering geometry when the reference point is located at the center of the rear wheel ($\mathcal B$).}\label{fig:rsteer_rear_ref}
% \end{figure}





% \subsection{Reference point at the center of gravity}
% Consider the bicycle model geometry in Figure \ref{fig:rsteer_cg_ref} that shows the reference point location at the center of gravity of the bicycle model. Let the coordinates of the reference point be $\mathcal C \equiv (x_c,y_c)$. On the four wheeled robot, this point corresponds to the center of gravity on the longitudinal axis of the robot. The direction of motion at $\mathcal{B}$ is at an angle $\bm{\beta}$ with respect to the longitudinal axis. $\bm{\beta}$ is called the slip angle. To derive the state gradient equations for the bicycle model, we consider $\triangle \mathcal{FIC}$ and $\triangle \mathcal{FIB}$. The slip angle $\bm{\beta}$ at the reference point $\mathcal C$ can be calculate as follows:

% \begin{flalign}
% &\tan{\delta} = \frac{\rm{L}}{\rm{R_{1}}} ~~ \Rightarrow ~~ \rm{R_{1}} = \frac{\rm{L}}{\tan{\delta}}\label{eq:cgref_tand}\\
% &\tan{\bm{\beta}} = \frac{\rm{L_{R}}}{\rm{R_{1}}} ~~ \Rightarrow ~~ \rm{R_{1}} = \frac{\rm{L_{R}}}{\tan{\bm{\beta}}}\label{eq:cgref_tanb}
% \end{flalign}

% \noindent Using equations (\ref{eq:cgref_tand}) and (\ref{eq:cgref_tanb}),
% \begin{flalign}
% &\frac{\rm{L}}{\tan{\delta}} = \frac{\rm{L_{R}}}{\tan{\bm{\beta}}}~~\Rightarrow~~\bm{\beta} = \arctan \left( \frac{\rm{L_{R}}}{\rm{L}}\tan{\delta} \right)
% \end{flalign}

% \noindent The turn radius R at the reference point $\mathcal C$ may be calculate using equation (\ref{eq:cgref_tand}) as follows:
% \begin{flalign}
% &\cos{\bm{\beta}} = \frac{\rm{R_{1}}}{\rm{R}} ~~ \Rightarrow ~~ \rm{R} = \frac{\rm{R_{1}}}{\cos{\bm{\beta}}} = \frac{\rm{L}}{\tan{\delta}\cos{\bm{\beta}}}
% \end{flalign}

% \noindent We can now write the equations for the state gradient as follows:
% \begin{flalign}
% &\dot x = v\cos{(\theta+\bm{\beta})}\\
% &\dot y = v\sin{(\theta+\bm{\beta})}\\
% &\dot \theta  = -\omega = -\frac{v}{\rm{R}} ~ = ~ -\frac{v}{\rm{L}}\tan{\delta}\cos{\bm{\beta}}
% \end{flalign}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\columnwidth,clip]{images/rsteer_cg_ref_newsymb.png}
%     \caption{Bicycle model for a rear steered vehicle with front wheel drivetrain. The figure shows the steering geometry when the reference point is located at the center of gravity of the robot ($\mathcal C$).}\label{fig:rsteer_cg_ref}
% \end{figure}



==> related_work_v0.tex <==
%auto-ignore
\section{Related Work}
In this section, we present a literature survey on the state of the art in agricultural robots, with an emphasis on weed control. Existing work on agricultural robots for weed control can be grouped into three broad categories: a) robot design, b) planning and navigation, and c) crop/weed detection. Since our work relates to robot design, specialized to particular environmental conditions, and planning and navigation within agricultural fields, we focus on these two categories in our literature review. Many design considerations and operational constraints for agricultural robots remain consistent across different applications. We present relevant work from the literature and discuss the placement of our work in context of the state of the art {\color{red}[to be done]}.

\subsection{Robot Design}
There are two common approaches to design autonomous mobile robots for operating in agricultural fields. The first approach is to custom-design the robot and build from ground up \cite{thorvald1,thorvald2,bawdenAGBOT}, and the second approach is to use an existing mobile platform and modify it to application requirements \cite{cv_pp_apples,BARTH201671,ball2016jfr}. The design process also includes the design and control of agricultural implements and/or end-effectors. Based on a particular application, the size and scale of the end-effector can vary from precise grippers for fruit picking to mowing implements weighing upwards of 250 kilograms. Grimstad et al. \cite{thorvald1,thorvald2} present a detailed analysis of system requirements and constraints to deploy an autonomous robot in agricultural fields. They present the design and demonstrate a prototype for their agricultural robot. They develop a modular and relatively light weight robot, marked with a payload capacity of 200 kilograms that can be configured to operate in a variety of environments. Bawden et. al. \cite{bawdenAGBOT} discuss the design of a versatile agricultural robot equipped with a heterogeneous set of weeding implements, and develop weed detection and classification methods based on local binary patterns and covariance features. Pérez-Ruíz et al. \cite{PEREZRUIZ201445} develop a human-operated semi-autonomous weeding robot for intra-row weeds. Hayashi et. al. \cite{cv_pp_strawberry} and Silwal et. al. \cite{cv_pp_apples} present the design of a strawberry harvesting robot and an apple harvesting robot, respectively. Hayashi et. al. use a suction based end-effector mounted on a custom platform while Silwal et al. employ an underactuated tendon-driven gripper mounted on a manually driven utility vehicle. Both works present a similar pipeline to detect and localize fruits, and then plan a path for the robotic manipulator to pluck them. Barth et al. \cite{BARTH201671} discuss an eye in hand configuration and present a software framework based on existing tools and libraries. They demonstrate the utility of their manipulator arm in a sweet pepper harvesting use case. Meuller-Sim et al. \cite{7989418} build a custom-designed robot and manipulator for contact based under-canopy phenotyping. In the case of Cowbot, we opted to build on top of an existing tractor platform that is engineered to perform well in rough outdoor environments and can operate heavy weeding implements weighing more than 250 kilograms.

%


% The robot designs and capabilities presented in \cite{thorvald2} (Thorvald ii) and \cite{bawdenAGBOT} (AGBOTII), are the state of the art in custom-built agricultural robots. Both robots have a versatile design for use in different environments and support a variety of agricultural implements for different tasks, including weed control.

%  They demonstrate the capabilities of their robot in a wide range of configurations and environments.

\subsection{Planning and navigation}
Path planning and navigation for agricultural robots is hard due to the difficult terrain and other uncontrolled natural factors. There is a strong body of literature on designing methods to enable autonomous robots to operate efficiently in agricultural fields. In particlar, Reina et al. \cite{REINA2016114,REINA2017124} address the terrain classification problem for operating agricultural robots. They evaluate the performance of complimentary sensor combinations and design a classifier to identify ploughed, unploughed, gravel and dirt road terrain types. Huang et. al. \cite{image_based_pp} develop path planning algorithms for a mobile ground robot to navigate in natural terrains. They design an approach to learn a color-to-cost mapping of the terrain and then use a pixel-to-pixel path search to find a traversable path. Hansen et. al. \cite{HANSEN2013217} develop vision based methods to detect weeds (thistles) on a sugar beet farm using aerial and ground robots, and use a genetic algorithm to compute tours for the ground robot. Evert et al. \cite{evert2011jfr} present the design of a custom designed robotic weeder to detect and control broad-leaved dock in grassland, and demonstrate the capabilities of their robot in field experiments. They present a behavior-based navigation controller to enable path following along straight lines and circular arcs. Hameed et. al. \cite{HAMEED201636} develop a path planning algorithm to minimize skips or overlap between adjacent passes for an agricultural robot due to altitude and/or terrain variability.

Since most commercial crops are grown in rows, row following \cite{ball2016jfr,MALAVAZI201871,BAKKEN2019102,BAYAR2016149} is a common requirement in the path planning module in agricultural robots. We give a brief overview of some recent work in this domain. Ball et al. \cite{ball2016jfr} develop an agricultural robot platform to perform coverage planning in row crops with vision based obstacle detection. They build on existing work in row tracking and path planning, and present details on system integration. They demonstrate day and night field operations of their robot. Malavazi et al. \cite{MALAVAZI201871} also address the navigation problem for an autonomous robot within rows, using LiDAR data. They design a robust data-fitting algorithm and use geometric priors to detect rows corresponding to dense point clouds on the field. Bakken et al. \cite{BAKKEN2019102} develop an end-to-end learning system for autonomous row following, with limited success. They train a convolutional neural network to output steering angle based on the current view of the environment and present results from preliminary field experiments for classifier and regression models. Bayar et al. \cite{BAYAR2016149} worked on improving the trajectory tracking performance of autonomous agricultural robots between rows of trees in an orchard. They design a model-based Lyapunov controller for path following along straight lines and circular arcs with wheel slip compensation.


\subsection{Robotic Weed Control}
The design of robotic weed management solutions has been studied extensively \cite{evert2011jfr}, \cite{thorvald1,thorvald2,bawdenAGBOT,PEREZRUIZ201445,lee1999robotic,OBERTI2016203,GONZALEZDESOTO2016165,agriculture9010018} and many different methods have been proposed to remove or kill weeds. We review different ways of robotic weed control in agriculture. In one of the early works on the design of robotic weeders, Lee et al. \cite{lee1999robotic} developed an intra-row chemical-spray robot. They present the construction of a precision spray system and an image processing pipeline to detect weeds in tomato crops. More recently, Oberti et al. \cite{OBERTI2016203} and Gonzalez-de-Soto et al. \cite{GONZALEZDESOTO2016165} present solutions for selective spraying for disease and weed control, respectively. Evert et al. \cite{evert2011jfr} present design considerations for their custom weeding robot with a rotating knife mechanism that drills weeds into the ground to kill them. Reiser et al. \cite{agriculture9010018} present the design of a robot, equipped with a rotary tiller mounted horizontally on a movable extended arm, for intra-row weeding. They evaluate the use of an electromechanical feeler and a sonar sensor to detect crop plants and move the weeding implement away from the row. Machleb et al. \cite{MACHLEB2020105638} present an excellent review of sensor-based weed control methods developed for agriculture. We refer the interested reader to the survey paper for a more exhaustive review.

% a selected set of work that comprises

%  More recently, Oberti et al. \cite{OBERTI2016203} present a solution for selective spraying of grapevines for disease control using a custom designed platform. They present the design of a manipulator arm, spray nozzle mechanism and disease detection mechanism using multispectral imagery with image processing techniques. Gonzalez-de-Soto et al. \cite{GONZALEZDESOTO2016165} develop an automated spray-system for precise spraying of weeds in an agricultural field. They present a system design to selectively activate the spray nozzles at known weed locations while also adjusting the dosage of herbicide. Controlled field experiments are presented to show proof-of-concept of the system.

==> sim_results_v0.tex <==
%auto-ignore
\section{Simulation Results}\label{ssec:sim_results}
% \begin{enumerate}
%     \item Baselines: algorithms and results
%     \item Simulation instances and new path planner performance
%     \item Results: plots and analysis
%     \item Effect of spatial weed density: simulated experiments
%     \item safety practices, hazops
% \end{enumerate}

To evaluate the performance of online planning algorithms presented in Section \ref{sec:sol_methods} we simulate the pasture environment and an autonomous mower operating on the pasture. The simulator was implemented using Python programming language and uses Robot Operating System (ROS) to mimic real-time communication on robot hardware. The simulations were run on a desktop computer with AMD Ryzen 7 processor and 32GB RAM. %The algorithms were also implemented in Python and were evaluated against a boustrophedon coverage path as baseline solution.

We benchmark the performance of the online algorithms using two baselines. First, the boustrophedon coverage path (referred as BCP) used to compute upper bounds on the path length for MRP as given in Section \ref{sec:sol_bounds}. We recall that path length in case of BCP is independent of the weed density and distribution on the pasture and is determined by the size of the pasture and the mower's parameters. For the second baseline, we modify the lower bounding boustrophedon coverage path given in Section \ref{sec:sol_bounds}. At the end of the coverage path, the mower has deterministic information about weeds and their locations within the pasture. We modify the algorithm to include a traveling salesman tour for the mower at the end of the boustrophedon path to visit each of the weeds detected on the pasture. We refer to this baseline as FOV-TSP.

\subsection{Simulation Setup} \label{sec:sim_setup}
We perform the simulations in a pasture of size 100m $\times$ 40m. The choice of pasture size ($\sim$ one acre) was made to be representative of the typical size of a paddock or a small pasture used for grazing cows. To populate weeds on the pasture, we use two different spatial distributions, uniform ($U$) and Gaussian ($G$). In the case of Gaussian distribution, 20\% of the weeds were sampled uniformly at random and were chosen as seeds for Gaussian clusters used to generate rest of the weed locations. Figures \ref{fig:jumppathplots} and \ref{fig:snakepathplots} show simulation instances with weeds sampled from a uniform and a Gaussian distribution, respectively. The autonomous mower is configured to operate with a constant speed of 1 m/s and comprises of a front mounted weeding implement of length $\mathcal{B} = 2m$. We vary the number of weeds $W$ on the pasture (in turn the weed density), the detection FOV and turning radius of the mower to study their effect on the length of the path computed by the online planners. For each combination of weed distribution ($U/G$) and weed count $W$, we generated 100 different instances. Table \ref{tab:simParams} lists the names and range of values for each of the simulation parameters. Figures \ref{fig:jumppathplots} and \ref{fig:snakepathplots} show sample simulation instances and mower paths computed using each of the online planning algorithms. 



\begin{figure*}
\centering
\subfloat[JUMP-LOW]{\includegraphics[width = 0.33\linewidth]{sim_images/JumpLow-Path.eps}}
\subfloat[JUMP-HIGH]{\includegraphics[width = 0.33\linewidth]{sim_images/JumpHigh-Path.eps}}
\subfloat[FOV-TSP]{\includegraphics[width = 0.33\linewidth]{sim_images/FovTSP-Path.eps}}
\caption{Mower paths planned using JUMP (a and b) online planning algorithm and FOV-TSP (c) baseline algorithm. The simulated pasture environment shows weed population sampled from a uniform distribution.}
\label{fig:jumppathplots}
\end{figure*}

\begin{figure*}
\centering
\subfloat[SNAKE-STATIC]{\includegraphics[width = 0.33\linewidth]{sim_images/SnakeStatic-Path.eps}}
\subfloat[SNAKE-STATIC-LIMITED]{\includegraphics[width = 0.33\linewidth]{sim_images/SnakeStaticLimited-Path.eps}}
\subfloat[SNAKE-DYNAMIC]{\includegraphics[width = 0.33\linewidth]{sim_images/SnakeDynamic-Path.eps}}
\caption{Mower paths planned using variants of the SNAKE online planning algorithm. The simulated pasture envrionment shows weed population sampled from a Gaussian distribution.}
\label{fig:snakepathplots}
\end{figure*}

\begin{table}[]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter} & \textbf{Values} \\ \hline
minimum turn radius: $\mathcal{R}$(m) &\{1,2,3,4,5\}  \\ \hline
depth of detection FOV: $\mathcal{S}_d(m)$ &\{4,8,12,16,20\} \\ \hline
width of detection FOV: $\mathcal{S}_w(m)$ &\{4,8,12,16,20\}  \\ \hline
\# of weeds: $W$ &\{20,40,80,160,320\}\\ \hline
\end{tabular}}
\caption{Range of values of various simulation parameters.}
\label{tab:simParams}
\end{center}
\end{table}

\subsection{Results}

% We perform four set of experiments varying each of the four simulation parameters in turn. Table \ref{tab:expParams} lists the combinations of parameter values used in each of the four experiments. 

We use two evaluation metrics to compare the solutions methods - a). length of the mower's path and b). percentage of weeds mowed on the pasture. For ease of exposition we express the path length as a percentage of the BCP path length. Figure \ref{fig:pathlength_vs_weeds} plots the aggregated length of the paths computed by the planning algorithms as a function of the number of weeds on the pasture. It plots the length of the paths on pastures for both uniform and Gaussian weed distributions. We observe that the path length needed to mow weed populations following different spatial distributions remains the same across algorithms. The number of weeds on the other hand visibly affects the path length: it increases consistently with increase in the number of weeds. Clearly, variants of the Snake algorithm perform better than the Jump algorithms in terms of path length and SSL outperforms all of the other algorithms. We also observe that the path length for all of the online planning algorithms converges to a value less than or equal to the BCP path length. Figure \ref{fig:weedsmowed_vs_weeds} plots the percentage of weeds mowed by the mower against the number of weeds in the pasture. It shows the trade-off to the shortest path length for SSL algorithm. At more than 95\% weed coverage, the SSL algorithm is still the lowest ranked amongst all algorithms. Meanwhile, the Jump algorithms achieve the highest weed coverage rate at 99.99 \%. These observations are consistent with the algorithms. The Jump algorithms are conservative in their approach and ensure that weeds are mowed on the pasture, even at the cost of longer paths for the mower. The Snake algorithms on the other hand generate consistently shorter paths but can miss a few weeds on the pasture. In conjunction, these algorithms provide a wide spectrum of choices to plan paths for an autonomous mower based on the trade-off between path length ($\simeq$ operating costs) and mowing efficiency. 


% FOV-TSP reduces to the lower bounding coverage path when there are no weeds on the pasture. However SSL starts to outperform the baseline algorithm as the weed density on the pasture start to increase.

%Path length for the FOV-TSP baseline algorithm increases linearly with increase in the number of weeds and even results in paths longer than COV-B.

% \begin{table}[]
% \begin{center}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  \textbf{Parameter} & \textbf{Experiment 1}& \textbf{Experiment 2}& \textbf{Experiment 3} & \textbf{Experiment 4} \\ \hline
%  $\mathcal{R}$ &2&\{1,2,3,4,5\} &2&2  \\ \hline
%  $\mathcal{S}_d$ &12&12&\{4,8,12,16,20\}&12  \\ \hline
%  $\mathcal{S}_w$ &12&12&12&\{4,8,12,16,20\}  \\ \hline
%  $W$ &\{20,40,80,160,320\}&\{40, 160, 320\}&\{40, 160, 320\}&\{40, 160, 320\}\\ \hline
% \end{tabular}}
% \caption{Parameter combinations used in the simulations.}
% \label{tab:expParams}
% \end{center}
% \end{table}

\begin{figure}
\centering
\subfloat[]{\includegraphics[width=0.49\linewidth]{sim_images/stepPercentage.png}\label{fig:pathlength_vs_weeds}}
\hspace{0cm}
\subfloat[]{\includegraphics[width=0.49\linewidth]{sim_images/weedsMowed.eps}\label{fig:weedsmowed_vs_weeds}}
\caption{(a) Mower path length (as \% of COV-B path length) vs number of weeds on the pasture. Solid lines represent path length in pastures with weeds sampled from a uniform distribution while dotted lines represent weeds sampled from a Gaussian distribution. (b) Percentage of weeds mowed by the mower vs number of weeds on the pasture.}
\end{figure}


\begin{figure*}
\centering
\subfloat[Effect of detection FOV depth ($\mathcal{S}_d$)]{\includegraphics[width = 0.33\linewidth]{sim_images/160.0Sdpercentage.eps}}
\subfloat[Effect of detection FOV width ($\mathcal{S}_w$)]{\includegraphics[width = 0.33\linewidth]{sim_images/160.0Swpercentage.eps}}
\subfloat[Effect of mower turn radius]{\includegraphics[width = 0.33\linewidth]{sim_images/160.0turnRpercentage.eps}}
\caption{Effect of varying mower's parameters' on path length.}
\label{fig:snakepathplots}
\end{figure*}

% The goal of the simulations is to show the efficiency of the proposed online planner algorithms for the mower routing problem. Therefore, we expect the online algorithms to navigate the mower on the pasture in a way that reduces the total path length relative to the offline baseline algorithms; without leaving unmowed weeds on the pasture. We generate pasture instances in simulation for dairy pastures that contain weeds to be mowed. Size of the pasture ($L \times B$) is fixed at one acre = 40m $ \times$ 100m. During initial experiments on the field using boustrophedon mowing paths, we found that the spatial distribution of weeds on a pasture is hard to characterise. However, to account for this, we still consider two different methods to generate weed locations within the pasture. First method generates weeds by sampling locations uniformly at random within the pasture and is represented by $\mathcal{U}$. The second method generates a small number of seeds within the pasture. The  weed  locations  are  then  sampled  from  within  the  Gaussian clusters initialized at a randomly chosen seed location and is represented by $\mathcal{N}$. The rate of randomly chosen seed locations is 20\% of the total weed count of an instance. The blade width ($\mathcal{B}$) of the mower is fixed at 2m for all the experiments and the mower moves with a fixed velocity ($\mathcal{V}$) of 1m. At the beginning of each instance, the mower always has a heading value of 0 rad. The fixed values for these parameters are also listed on Table \ref{tab:fixedParams}. Minimum turn radius of the mower $\mathcal{R}$, depth of detection footprint $\mathcal{S}_d$, width of detection footprint $\mathcal{S}_w$ and number of weeds on $\mathcal{E}$ were varied as simulation parameters. The values for each of the parameters are listed on Table \ref{tab:testParams}.

% We evaluate the quality of every algorithm according to the following 3 criteria: The length of the path covered by the mower, measured relative to the offline boustrophedon path covering an instance. The percent of weeds detected by the mower. The percent of weeds mowed by the mower. The percentage of weeds is relative to the total number of weeds on $\mathcal{E}$ for an instance.

% All 5 of proposed algorithms are tested against 2 TSP based baseline algorithms, over a set of 4 different experiment groups. Each experiment's independent variables are presented on Table \ref{tab:testParams}. Different instances within an experiment set each represent a different  randomly sampled weed distribution whereas experiments sharing the same number of weeds on $\mathcal{E}$ value also share the same set of instances. The first experiment is for observing each algorithm's behaviour with respect to changes in number of weeds on $\mathcal{E}$. Since the offline boustrophedon algorithm's behavior does not depend on the weeds on $\mathcal{E}$, we expect the online algorithms' path length to increase significantly with increasing number of weeds. In the second experiment, $\mathcal{R}$ is changed and the algorithms' performances are observed. $\mathcal{R}$ is a parameter that determines the length of the Dubins paths, therefore we expect an increase in $\mathcal{R}$ to make online algorithms' paths longer. The third and fourth experiments are for observing the algorithms' performances with respect to $\mathcal{S}_d$ and $\mathcal{S}_w$, respectively. Generally, an increase in those values is expected make the algorithm to plan online more efficiently, hence the path length is expected to decrease.

% \subsection{Results}

% Results for the first experiment are shown on Figure XYZ. Figure XYZa shows the total path length of the mower plotted against an increasing number of weeds as shown on Table \ref{tab:testParams}, Experiment 1 column. It is observed from the figure that an increase in number of weeds increases the total path length. It is also observable that this trend can reach a level where the algorithms lose their relative advantages against the offline boustrophedon planner. Figures XYZ quantify the missed pasture coverage in terms of weeds and we measure the percentage of weeds left undetected or unmowed. For Experiment 1, all the algorithms achieve detection and mowing rates above 95\% and the JumpLow algorithm achieves 100\% mowing rate. Since it is trivial to show that the boustrophedon path blade coverage algorithm's behaviour will be the same within experiment groups except for the second test group, its behaviour is excluded from the plots.

% Path length results for the second, third and fourth experiments are shown on Figures XYZabc for 160 weeds. For Experiment 2, Figure XYZa shows the total path length of the mower plotted against the parameter $\mathcal{R}$ and it shows that an increase in $\mathcal{R}$ also increases the path length for the online planners except for SnakeStaticLimited. For Experiment 3, Figure XYZb visualizes the total path length of the mower plotted against the parameter $\mathcal{S}_d$. Experiment 3 shows that the path length decreases slightly if we increase $\mathcal{S}_d$. For Experiment 4, Figure XYZc shows the total path length of the mower plotted against the parameter $\mathcal{S}_w$. Experiment 4 shows that increasing $\mathcal{S}_w$ helps the Snake planners, but actually increases the total path length of the Jump planners after 8m.

% Figures \ref{fig:baselinepathplots}, \ref{fig:jumppathplots} and \ref{fig:snakepathplots} show sample paths generated by these algorithms on randomly generated pastures containing 20 weeds with $\mathcal{U}$ distribution. The turn radius ($\mathcal{R}$) for the mower used for generating these paths is 5m. The depth ($\mathcal{S}_d$) and the width ($\mathcal{S}_w$) of detection footprint are equal and 10m. The pasture size ($L \times B$) is 40m $\times$ 100m. 

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/stepPercentage.eps}
% \caption{Path length divided by the corresponding boustrophedon path length, with respect to number of weeds}\label{fig:stepPerc}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/weedsDetected.eps}
% \caption{Percentage of weeds detected, with respect to number of weeds}\label{fig:weedsDet}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/weedsMowed.eps}
% \caption{Percentage of weeds mowed, with respect to number of weeds}\label{fig:weedsMow}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/160.0turnRpercentage.eps}
% \caption{Path length divided by the corresponding boustrophedon path length}\label{fig:160turnrperc}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/160.0Sdpercentage.eps}
% \caption{Path length divided by the corresponding boustrophedon path length}\label{fig:160sdperc}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{burak_plots/160.0Swpercentage.eps}
% \caption{Path length divided by the corresponding boustrophedon path length}\label{fig:160swperc}
% \end{figure}




% \begin{table}[]
% \begin{center}
% \begin{tabular}{|c|c|}
% \hline
%  \textbf{Parameter Name} & \textbf{Values} \\ \hline
%  $L \times B$ & 100m x 40m \\ \hline
%  \# instances & 100 \\ \hline
%  weed distribution type & $\mathcal{U}$ or $\mathcal{N}$  \\ \hline
%  $\mathcal{B}$ & 2.0m \\ \hline
%  $\mathcal{V}$ & 1.0 \\ \hline
%  initial heading(rad) & 0 \\ \hline
%  Gaussian seed rate & 20\% \\ \hline
% \end{tabular}
% \caption{Fixed parameters used in the simulated experiments.}
% \label{tab:fixedParams}
% \end{center}
% \end{table}


% \begin{table}[]
% \begin{center}
% \scalebox{0.65}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  \textbf{Parameter} & \textbf{Experiment 1}& \textbf{Experiment 2}& \textbf{Experiment 3} & \textbf{Experiment 4} \\ \hline
%  minimum turn radius: $\mathcal{R}$(m) &2&\{1,2,3,4,5\} &2&2  \\ \hline
%  depth of detection footprint: $\mathcal{S}_d(m)$ &12&12&\{4,8,12,16,20\}&12  \\ \hline
%  width of detection footprint: $\mathcal{S}_w(m)$ &12&12&12&\{4,8,12,16,20\}  \\ \hline
%  number of weeds on $\mathcal{E}$&\{20,40,80,160,320\}&\{40, 160, 320\}&\{40, 160, 320\}&\{40, 160, 320\}\\ \hline
% \end{tabular}}
% \caption{Parameters used in the simulated experiments.}
% \label{tab:testParams}
% \end{center}
% \end{table}

% \begin{figure}
% \centering
% \subfloat[Coverage TSP algorithm path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/FovTSP-Path.eps}}\\
% \subfloat[A priori TSP algorithm path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/FullTSP-Path.eps}}\\
% \caption{Baseline algorithms' paths}
% \label{fig:baselinepathplots}
% \end{figure}

% \begin{figure}
% \centering
% \subfloat[JUMP-LOW path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/JumpLow-Path.eps}}\\
% \subfloat[JUMP-HIGH path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/JumpHigh-Path.eps}}\\
% \caption{JUMP algorithms' paths}
% \label{fig:jumppathplots}
% \end{figure}

% \begin{figure}[h]
% \centering
% \subfloat[SNAKE-DYNAMIC path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/SnakeDynamic-Path.eps}}\\
% \subfloat[SNAKE-STATIC path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/SnakeStatic-Path.eps}}\\
% \subfloat[SNAKE-STATIC-LIMITED path]{\includegraphics[width = 3.25in]{burak_plots/full_path_plots/SnakeStaticLimited-Path.eps}}\\
% \caption{SNAKE algorithms' paths}
% \label{fig:snakepathplots}
% \end{figure}

% \iffalse
% \subsection{Field Data}
% How is it collected? Maybe picture? All algos work fine here except SnakeStaticLimited. Parameters: fov = [12, 12], turnR = 2, LxB = 23, 43, 33 weeds.



% \begin{figure}[h]
% \centering
% \subfloat[Field-FOVTSP path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/fovtsp.eps}}\\
% \subfloat[Field-FULLTSP path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/fulltsp.eps}}\\
% \caption{Baseline algorithms' field paths}
% \label{fig:geotaggedbaselineplots}
% \end{figure}
% \fi

% \begin{figure}[h]
% \centering
% \subfloat[Field-JumpHigh path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/field_jh_path.eps}}\\
% \subfloat[Field-JumpLow path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/field_jl_path.eps}}\\
% \caption{Jump algorithms' field paths}
% \label{fig:geotaggedjumpplots}
% \end{figure}

% \begin{figure}[h]
% \centering
% \subfloat[Field-SnakeDynamic path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/field_sd_path.eps}}\\
% \subfloat[Field-SnakeStatic path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/field_ss_path.eps}}\\
% \subfloat[Field-SnakeStaticLimited path]{\includegraphics[width = 3.25in]{burak_plots/field_path_plots/field_ssl_path.eps}}\\
% \caption{Snake algorithms' field paths}
% \label{fig:geotaggedsnakeplots}
% \end{figure}

% \subsection{Discussion}
% \begin{itemize}
%     \item Main argument is that proposed algorithms save steps compared to boustrophedon coverage.
%     \item However beyond a certain weed density, it is just more feasible to do a boustrophedon full pass.
%     \item Gaussian and Uniform distributions do not change much.
%     \item Experimentally, JUMP-LOW does not miss any weeds, the rest also have very good coverage except SNAKESTATIC-LIMITED
%     \item Present behaviour of all vs weed Density and then present the rest of the plots on 160 weeds. Justify the 160 weeds decision. Mention the limited algorithm stays low steps percentage.
% \end{itemize}

==> snake_planner_v0.tex <==
%auto-ignore
\subsection{SNAKE Online Planning Algorithm}
The SNAKE planner derives its name from the curvy serpentine-like patterns generated in paths computed by the planner. The algorithm generates to and fro passes across the pasture, similar to a boustrophedon path, while also utilizing the agility of a Dubins' motion model to design efficient paths for the mower. %It uses a variable sized plsn window to generate a path for the mower. 

Consider the mower's traversal along a pass of the boustrophedon coverage path through the pasture. The list of weeds, $\mathcal{W}$, maintained by the mower comprises of all weeds detected so far in the pasture that are yet to be mowed. At each time step the planner checks for weeds, $w_i \in \mathcal{W}$, that satisfy the following set of constraints:
\begin{align*}
\mathcal{F}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
&x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
&y_i < y_p+\mathcal{S}_w/2&
\end{align*}
Let $\mathcal{W}_f$ be the list of weeds that satisfy the constraint set $\mathcal{F}$. The weeds in $\mathcal{W}_f$: 1) lie ahead of the mower in the direction of its motion, and 2) lie below the upper limit of the detection field of view of the mower on the current pass.

The planner considers the weeds, $w_k \in \mathcal{W}_f$, in the increasing order of their distance from the mower along its direction of motion on the current pass i.e. $\|x_m - x_k\|$. It then computes a sub-path for the mower to reach the location of the first weed in the sorted list with heading angle $\theta_p$. For sub-path computation, if $\theta_p=0$ the SNAKE planner only considers Dubins paths of type LSR for weeds located above $y_m$ and of type RSL for weeds located below $y_m$. If $\theta_p=\pi$, the planner only considers Dubins paths of type RSL for weeds located above $y_m$ and of type LSR for weeds located below $y_m$ for sub-path computation. If a valid sub-path of the requisite type is not available to the first weed on the list, the planner skips to the next weed until it finds a valid sub-path or reaches the end of the list. When the planner finds a valid sub-path, the mower starts executing it. We refer to the execution of a sub-path by the mower as a wriggle action. While the mower wriggles to a weed, the planner does not search for new sub-paths. When the mower reaches the end of a sub-path and mows the corresponding weed, the planner resumes its search for the next sub-path. If $\mathcal{W}_f$ is empty or there does not exist a valid sub-path to any of the weeds in $\mathcal{W}_f$, the mower continues to move straight ahead with heading $\theta_m = \theta_p$ and repeats its search for sub-paths to weeds in $\mathcal{W}_f$ at the next time step.

Note that, there isn't a lower limit on the y-coordinate value for weeds in $\mathcal{W}_f$. We define another set of constraints $\mathcal{F}'$ that comprises of all constraints in the set $\mathcal{F}$ and additionally Eq. \ref{eq:snake_wf_lb}.
\begin{align}
&y_i > y_p-\frac{3}{2}\mathcal{S}_w& \label{eq:snake_wf_lb}
\end{align}
The constraint set $\mathcal{F}'$ imposes a lower limit on the y-coordinate value of weeds in the set $\mathcal{W}_f$. Since the mower can wriggle up or down on a sub-path, this constraint restricts the maximum downward movement of the mower to mow a weed. We use the constraint set $\mathcal{F}'$ later in the text to develop variants of the SNAKE algorithm.

At the end of a pass, the planner computes $y_p$ value for the next pass with $\theta_p = \pi - \theta_p$. We present two methods to compute the $y_p$ value. The first method uses a fixed spacing between passes while the second method uses dynamic spacing similar to the JUMP algorithm. The $y_p$ value for the next pass, with fixed spacing, is calculated as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    y_p(i)+\mathcal{S}_w/2 + \mathcal{B}/2\\
    B - \mathcal{B}/2
    \end{cases}\label{eq:yp_compute_snake_fixed}
\end{align}
 The $y_p$ value for the next pass, with dynamic spacing, is calculated as follows:
\begin{align}
    y_p(i+1)&  = \rm{min}
    \begin{cases}
    \min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2+\mathcal{B}/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:yp_compute_snake_dynamic}
\end{align}


\begin{algorithm}
\caption{SNAKE-planner}\label{algo:snakeAlgo}
\begin{algorithmic}[1]
\Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
\Statex $\mathcal{I}$: vector of 1s
% \Statex
\State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2\Comment{y value corr. to current pass}
\State $\theta_p = 0$\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]\Comment{weed list}
\State mission\_completed = False \Comment{termination flag}
\State wriggle\_flag = 0 \Comment{0: not wriggling, 1: wriggling}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  initial\_pose \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}
\State current\_path = [$0:L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$L:0$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{not reached end of pass}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{wriggle\_flag == 1}
\State take next step on  current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{wriggle is complete}
\State wriggle\_flag = 0
\If{$\theta_p$ == 0}
\State current\_path = [$x_m:L$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$x_m:0$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\EndIf
\State continue
\EndIf
\State $\Omega$ = find\_valid\_subpath()
\If{$\Omega$ is not empty}
\State current\_path = $\Omega$
\State wriggle\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{termination condition is true}
\State mission\_completed = True
\State continue
\EndIf
% \Statex
\State Compute new value of $y_p$ for next pass
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}



We are now ready to define the three variants of the SNAKE algorithm. The first variant called SNAKE-STATIC (SS) uses a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). fixed spacing between passes (Eq \ref{eq:yp_compute_snake_fixed}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
\end{align}
The second variant called SNAKE-STATIC-LIMITED (SSL) uses a). constraint set $\mathcal{F}'$ to compute $\mathcal{W}_f$, b). fixed spacing between passes (Eq \ref{eq:yp_compute_snake_fixed}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_static_limited}
\end{align}

The third variant called SNAKE-DYNAMIC (SD) uses a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). dynamic spacing between passes (Eq \ref{eq:yp_compute_snake_dynamic}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
\end{align}






% At the end of a pass, the planner computes $y_p$ for the next pass with $\theta_p = \pi - \theta_p$. We present two methods to compute the $y_p$ value, that lead to two different variants of the SNAKE algorithm. The first method uses a fixed spacing between passes. The $y_p$ value for the next pass, with fixed spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(y_p+\mathcal{S}_w/2 + \mathcal{B}/2, B - \mathcal{B}/2)\label{eq:yp_compute_snake_fixed}
% \end{align}
% Termination criteria for the first variant, evaluated at the end of each pass, is as follows:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
% \end{align}

% The second method uses dynamic spacing between passes, similar to the JUMP algorithm. The $y_p$ value for the next pass, with dynamic spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2), B-\mathcal{B}/2)\label{eq:yp_compute_snake_dynamic}
% \end{align}
% Termination criteria for the second variant, evaluated at the end of each pass, is
% \begin{align}
%     (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
% \end{align}

% We also present a third method that is a variant of the SNAKE-STATIC and is named SNAKE-STATIC-LIMITED. The $y_p$ value for the next pass is calculated the same way as the SNAKE-STATIC. This variant checks a slightly different set of constraints to be satisfied for weeds, $w_i \in \mathcal{W}$: 
% \begin{align*}
% \mathcal{F'}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
% &x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
% &y_i > y_p-1.5\mathcal{S}_w&\\
% &y_i < y_p+\mathcal{S}_w/2&
% \end{align*}

% Termination criteria for the third variant, evaluated at the end of each pass is:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_dynamic_limited}
% \end{align}


==> snake_planner_v1.tex <==
%auto-ignore
\subsection{SNAKE Online Planning Algorithm}
The SNAKE planner (Algorithm \ref{algo:snakeAlgo}) derives its name from curvy serpentine-like patterns generated in paths computed by the planner.  To explain the working of the planner, we consider the mower's traversal along a pass of the boustrophedon coverage path. At each time step the planner checks for weeds $w_i \equiv (x_i,y_i) \in \mathcal{W}$ that satisfy the criteria:
\begin{align*}
\mathcal{F}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
&x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
&y_i < y_p+\mathcal{S}_w/2&
\end{align*}
Let $\mathcal{W}_f$ be the list of weeds that satisfy the constraint set $\mathcal{F}$. The planner considers weeds, $w_k \in \mathcal{W}_f$, in the increasing order of their distance from the mower ($\|x_m - x_k\|$). It then computes a sub-path for the mower to reach the location of the first weed in the sorted list with heading angle $\theta_p$. For sub-path computation, if $\theta_p=0$ the SNAKE planner only considers Dubins paths of type LSR for weeds located above $y_m$ and of type RSL for weeds located below $y_m$. If $\theta_p=\pi$, the planner only considers Dubins paths of type RSL for weeds located above $y_m$ and of type LSR for weeds located below $y_m$. If a valid sub-path of the requisite type is not available to the first weed on the list, the planner skips to the next weed until it finds a valid sub-path or reaches the end of the list. When the planner finds a valid sub-path, the mower starts executing it. While the mower is executing a sub-path, the planner does not search for new sub-paths. When the mower reaches the end of a sub-path and mows the corresponding weed, the planner resumes its search for the next sub-path. If $\mathcal{W}_f$ is empty or there does not exist a valid sub-path to any of the weeds in $\mathcal{W}_f$, the mower continues to move straight ahead with heading $\theta_m = \theta_p$ and repeats its search for sub-paths to weeds in $\mathcal{W}_f$ at the next time step.

% Note that, there isn't a lower limit on the y-coordinate value for weeds in $\mathcal{W}_f$.
We define another set of constraints $\mathcal{F}'$ that comprises of all constraints in the set $\mathcal{F}$ and additionally Eq. \ref{eq:snake_wf_lb}.
\begin{align}
&y_i > y_p-\frac{3}{2}\mathcal{S}_w& \label{eq:snake_wf_lb}
\end{align}
% The constraint set $\mathcal{F}'$ imposes a lower limit on the y-coordinate value of weeds in the set $\mathcal{W}_f$. Since the mower can wriggle up or down on a sub-path, this constraint restricts the maximum downward movement of the mower to mow a weed. 
We use the constraint set $\mathcal{F}'$ later in the text to develop variants of the SNAKE algorithm.

At the end of a pass, the planner computes $y_p$ value for the next pass with $\theta_p = \pi - \theta_p$. We present two methods to compute the $y_p$ value. The first method uses a fixed spacing between passes while the second method uses dynamic spacing similar to the JUMP algorithm. $y_p$ value for the next pass, with fixed spacing, is calculated as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    y_p(i)+\mathcal{S}_w/2 + \mathcal{B}/2\\
    B - \mathcal{B}/2
    \end{cases}\label{eq:yp_compute_snake_fixed}
\end{align}
$y_p$ value for the next pass, with dynamic spacing, is calculated as follows:
\begin{align}
    y_p(i+1)&  = \rm{min}
    \begin{cases}
    \min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2\\
    y_p(i)+\mathcal{S}_w/2+\mathcal{B}/2\\
    B-\mathcal{B}/2
    \end{cases}\label{eq:yp_compute_snake_dynamic}
\end{align}


\begin{algorithm}
\caption{SNAKE-planner ($L,B,\mathcal{S}_d,\mathcal{S}_w,\mathcal{B},\mathcal{R}$)}\label{algo:snakeAlgo}
\begin{algorithmic}[1]
% \Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
% \Statex $\mathcal{I}$: vector of 1s
% \Statex
% \State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2%\Comment{y value corr. to current pass}
\State $\theta_p = 0$%\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]%\Comment{weed list}
\State mission\_completed = False %\Comment{termination flag}
\State wriggle\_flag = 0 %\Comment{0: not wriggling, 1: wriggling}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  \{$0,~\mathcal{B}$/2, 0\}% \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}\Comment{$\mathcal{I}$: vector of 1s}
\State current\_path = [$0:L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$L:0$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{$x_m < L$}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{wriggle\_flag == 1}
\State take next step on  current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{reached end of current\_path}
\State wriggle\_flag = 0
\If{$\theta_p$ == 0}
\State current\_path = [$x_m:L$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$x_m:0$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\EndIf
\State continue
\EndIf
\State $\Omega$ = find\_valid\_subpath()
\If{$\Omega$ is not empty}
\State current\_path = $\Omega$
\State wriggle\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{termination condition is true}
\State mission\_completed = True
\State \Return
\EndIf
% \Statex
\State Compute $y_p$ for next pass
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}



We are now ready to define the three variants of the SNAKE algorithm. The first variant called SNAKE-STATIC (SS) uses- a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). fixed spacing between passes (Eq \ref{eq:yp_compute_snake_fixed}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_m \geq B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
\end{align}
The second variant called SNAKE-STATIC-LIMITED (SSL) uses- a). constraint set $\mathcal{F}'$ to compute $\mathcal{W}_f$, b). fixed spacing between passes (Eq \ref{eq:yp_compute_snake_fixed}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_m \geq B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_static_limited}
\end{align}

The third variant called SNAKE-DYNAMIC (SD) uses- a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). dynamic spacing between passes (Eq \ref{eq:yp_compute_snake_dynamic}) and c). the following termination criteria, evaluated at the end of each pass:
\begin{align}
    (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
\end{align}






% At the end of a pass, the planner computes $y_p$ for the next pass with $\theta_p = \pi - \theta_p$. We present two methods to compute the $y_p$ value, that lead to two different variants of the SNAKE algorithm. The first method uses a fixed spacing between passes. The $y_p$ value for the next pass, with fixed spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(y_p+\mathcal{S}_w/2 + \mathcal{B}/2, B - \mathcal{B}/2)\label{eq:yp_compute_snake_fixed}
% \end{align}
% Termination criteria for the first variant, evaluated at the end of each pass, is as follows:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
% \end{align}

% The second method uses dynamic spacing between passes, similar to the JUMP algorithm. The $y_p$ value for the next pass, with dynamic spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2), B-\mathcal{B}/2)\label{eq:yp_compute_snake_dynamic}
% \end{align}
% Termination criteria for the second variant, evaluated at the end of each pass, is
% \begin{align}
%     (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
% \end{align}

% We also present a third method that is a variant of the SNAKE-STATIC and is named SNAKE-STATIC-LIMITED. The $y_p$ value for the next pass is calculated the same way as the SNAKE-STATIC. This variant checks a slightly different set of constraints to be satisfied for weeds, $w_i \in \mathcal{W}$: 
% \begin{align*}
% \mathcal{F'}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
% &x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
% &y_i > y_p-1.5\mathcal{S}_w&\\
% &y_i < y_p+\mathcal{S}_w/2&
% \end{align*}

% Termination criteria for the third variant, evaluated at the end of each pass is:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_dynamic_limited}
% \end{align}


==> snake_planner_v2.tex <==
%auto-ignore
\subsection{SNAKE Online Planning Algorithm}
The SNAKE planner (Algorithm \ref{algo:snakeAlgo}) derives its name from curvy to-and-fro serpentine patterns across the pasture generated in paths computed by the planner. It builds on a boustrophedon coverage path and we consider the mower's traversal along a pass of the boustrophedon path to explain the working of the planner. At each time step along the path the planner checks for weeds $w_i \equiv (x_i,y_i) \in \mathcal{W}$ that satisfy the following criteria:
\begin{align*}
\mathcal{F}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
&x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
&y_i < y_p+\mathcal{S}_w/2&
\end{align*}
Let $\mathcal{W}_f$ be the list of weeds that satisfy the constraint set $\mathcal{F}$. The planner considers weeds, $w_k \in \mathcal{W}_f$, in the increasing order of their distance from the mower ($\|x_m - x_k\|$). It then computes a sub-path for the mower to reach the location of the first weed in the sorted list with heading angle $\theta_p$.

For sub-path computation, we use primitives from the Dubins' shortest path algorithm for curvature constrained vehicle \cite{dubins}. Specifically we consider Dubins's paths of the type $C^+SC^-$, where $C^+$ and $C^-$ are circular arcs in opposite direction and $S$ is a straight line path. LSR and RSL paths are realizations of the $C^+SC^-$ path type, where R refers to a circular arc in the clockwise direction and L refers to a circular arc in the counter clockwise direction. If $\theta_p=0$ the SNAKE planner only considers Dubins paths of type LSR for weeds located above $y_m$ and of type RSL for weeds located below $y_m$. If $\theta_p=\pi$, the planner only considers Dubins paths of type RSL for weeds located above $y_m$ and of type LSR for weeds located below $y_m$. If a valid sub-path of the requisite type is not available to the first weed on the list, the planner skips to the next weed until it finds a valid sub-path or reaches the end of the list. When the planner finds a valid sub-path, the mower starts executing it. While the mower is executing a sub-path, the planner does not search for new sub-paths. When the mower reaches the end of a sub-path and mows the corresponding weed, the planner resumes its search for the next sub-path. If $\mathcal{W}_f$ is empty or there does not exist a valid sub-path to any of the weeds in $\mathcal{W}_f$, the mower continues to move straight ahead with heading $\theta_m = \theta_p$ and repeats its search for sub-paths to weeds in $\mathcal{W}_f$ at the next time step. At the end of each pass, the planner computes $y_p$ value for the next pass with $\theta_p = \pi - \theta_p$ as follows:
\begin{align}
    y_p(i+1) = \rm{min}
    \begin{cases}
    y_p(i)+\mathcal{S}_w/2 + \mathcal{B}/2\\
    B - \mathcal{B}/2
    \end{cases}\label{eq:yp_compute_snake_fixed}
\end{align}
Termination criteria for the SNAKE planner, evaluated at the end of each pass, is:
\begin{align}
    (y_m \geq B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
\end{align}


% Note that, there isn't a lower limit on the y-coordinate value for weeds in $\mathcal{W}_f$.

% The constraint set $\mathcal{F}'$ imposes a lower limit on the y-coordinate value of weeds in the set $\mathcal{W}_f$. Since the mower can wriggle up or down on a sub-path, this constraint restricts the maximum downward movement of the mower to mow a weed. 

We define another variant of the SNAKE planner called the RESTRICTED-SNAKE (R-SNAKE) that uses the constraint set $\mathcal{F}'$ to compute $\mathcal{W}_f$. $\mathcal{F}'$ comprises of all constraints in the set $\mathcal{F}$ and additionally Eq. \ref{eq:snake_wf_lb}.
\begin{align}
&y_i > y_p-\frac{3}{2}\mathcal{S}_w& \label{eq:snake_wf_lb}
\end{align}
R-SNAKE uses the following termination criteria evaluated at the end of each pass:
\begin{align}
    (y_m \geq B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_static_limited}
\end{align}

\begin{algorithm}
\caption{SNAKE-planner ($L,B,\mathcal{S}_d,\mathcal{S}_w,\mathcal{B},\mathcal{R}$)}\label{algo:snakeAlgo}
\begin{algorithmic}[1]
% \Statex Input: pasture $\equiv (L\times B)$, FOV $\equiv (\mathcal{S}_d,\mathcal{S}_w)$, $\mathcal{B}$, $\mathcal{R}$
% \Statex $\mathcal{I}$: vector of 1s
% \Statex
% \State initial\_pose =  \{$0,~\mathcal{B}$/2, 0\}
\State $y_p = \mathcal{B}$/2%\Comment{y value corr. to current pass}
\State $\theta_p = 0$%\Comment{heading direction of current pass}
\State $\mathcal{W}$ = [ ]%\Comment{weed list}
\State mission\_completed = False %\Comment{termination flag}
\State wriggle\_flag = 0 %\Comment{0: not wriggling, 1: wriggling}
% \State path\_f = [0 : $L$, step=$\delta$] \Comment{forward pass}
% \State path\_b = [$L$ : 0, step=$-\delta$] \Comment{backward pass}
\State current\_pose =  \{$0,~\mathcal{B}$/2, 0\}% \Comment{pose: $\{x_m,y_m,\theta_m\}$}
% \Statex
\While{mission\_completed is False}
\If{$\theta_p == 0$}\Comment{$\mathcal{I}$: vector of 1s}
\State current\_path = [$0:L$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$L:0$, $y_p.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\State transit\_path = dubins(current\_pose, current\_path[0])
\State current\_path.prepend(transit\_path)
% \Statex
\While{$x_m < L$}
\State add new weeds detected in current FOV to $\mathcal{W}$
\If{wriggle\_flag == 1}
\State take next step on  current\_path
\State remove mowed weeds from $\mathcal{W}$
\If{reached end of current\_path}
\State wriggle\_flag = 0
\If{$\theta_p$ == 0}
\State current\_path = [$x_m:L$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\ElsIf{$\theta_p == \pi$}
\State current\_path = [$x_m:0$, $y_m.\mathcal{I}$, $\theta_p.\mathcal{I}$]
\EndIf
\EndIf
\State continue
\EndIf
\State $\Omega$ = find\_valid\_subpath()
\If{$\Omega$ is not empty}
\State current\_path = $\Omega$
\State wriggle\_flag = 1
\EndIf
\State take next step on current\_path
\State remove mowed weeds from $\mathcal{W}$
\EndWhile
% \Statex
\If{termination condition is true}
\State mission\_completed = True
\State \Return
\EndIf
% \Statex
\State Compute $y_p$ for next pass
\State $\theta_p = \pi - \theta_p$
\EndWhile
\end{algorithmic}
\end{algorithm}


% The third variant called SNAKE-DYNAMIC (SD) uses- a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). dynamic spacing between passes (Eq \ref{eq:yp_compute_snake_dynamic}) and c). the following termination criteria, evaluated at the end of each pass:
% \begin{align}
%     (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
% \end{align}





% We are now ready to define the SNAKE algorithm. The SNAKE online planner uses- a). constraint set $\mathcal{F}$ to compute $\mathcal{W}_f$, b). fixed spacing between passes (Eq \ref{eq:yp_compute_snake_fixed}) and c). 




% At the end of a pass, the planner computes $y_p$ for the next pass with $\theta_p = \pi - \theta_p$. We present two methods to compute the $y_p$ value, that lead to two different variants of the SNAKE algorithm. The first method uses a fixed spacing between passes. The $y_p$ value for the next pass, with fixed spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(y_p+\mathcal{S}_w/2 + \mathcal{B}/2, B - \mathcal{B}/2)\label{eq:yp_compute_snake_fixed}
% \end{align}
% Termination criteria for the first variant, evaluated at the end of each pass, is as follows:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_fixed}
% \end{align}

% The second method uses dynamic spacing between passes, similar to the JUMP algorithm. The $y_p$ value for the next pass, with dynamic spacing, is calculated as follows:
% \begin{align}
%     y_p = \rm{min}(\min_{\forall i:w_i \in \mathcal{W}}y_i+\mathcal{B}/2, (y_p+\mathcal{S}_w/2+\mathcal{B}/2), B-\mathcal{B}/2)\label{eq:yp_compute_snake_dynamic}
% \end{align}
% Termination criteria for the second variant, evaluated at the end of each pass, is
% \begin{align}
%     (y_p==B-\mathcal{B}/2)~ \cap ~(\mathcal{W} == \phi)\label{eq:terminate_snake_dynamic}
% \end{align}

% We also present a third method that is a variant of the SNAKE-STATIC and is named SNAKE-STATIC-LIMITED. The $y_p$ value for the next pass is calculated the same way as the SNAKE-STATIC. This variant checks a slightly different set of constraints to be satisfied for weeds, $w_i \in \mathcal{W}$: 
% \begin{align*}
% \mathcal{F'}: ~~&x_i > x_m, ~~\rm{if}~\theta_p = 0&\\
% &x_i < x_m,~~ \rm{if}~\theta_p = \pi&\\
% &y_i > y_p-1.5\mathcal{S}_w&\\
% &y_i < y_p+\mathcal{S}_w/2&
% \end{align*}

% Termination criteria for the third variant, evaluated at the end of each pass is:
% \begin{align}
%     (y_m >= B - \mathcal{B})~ \cap ~(y_p == B - \mathcal{B}/2)\label{eq:terminate_snake_dynamic_limited}
% \end{align}


==> solution_v0.tex <==
%auto-ignore
\section{Solution Methods}\label{sec:sol_methods}

In this section, we present solution methods to the mower routing problem to detect and mow weeds on a pasture. We first describe common terminology used in the rest of the section. We then develop bounds on the solution space and present baseline solution methods. Following that we present the design and construction of two online planning algorithms, named SNAKE and JUMP.

% In this section, we present the design and construction of two online planning algorithms called JUMP and SNAKE, to solve the mower routing problem. In the following text, we describe details common to both planners. 

Given a rectangular pasture $\mathcal{E}$ of size ($L\times B$), we consider an inertial frame of reference such that the four corners of the pasture are located at $(0,0), (L,0), (L,B)$ and $(0,B)$. For ease of exposition we will refer to locations with bigger $y$-coordinate values as being located above locations with smaller $y$-coordinate values, and vice-versa as being located below. We use a triplet of the form $(x_m,y_m,\theta_m)$ to represent the current state of the mower in the pasture, where $(x_m,y_m)$ are the location coordinates and $\theta_m$ is the heading angle of the mower. The autonomous mower maintains a list, $\mathcal{W}$, of weeds detected on the pasture that are yet to be mowed. %When a new weed, $w_i=(x_i,y_i)$, is detected within the field of view of the mower, it is added to $\mathcal{W}$. Once the mower has mowed the weed, it is removed from $\mathcal{W}$.

% a longer edge is aligned with the x-axis, a shorter edge is aligned with the $y$-axis and the bottom left corner of the pasture is placed at $(0,0)$. T

% Consider a boustrophedon path to cover the pasture, such that the passes in the path are parallel to $x$-axis. The first pass is along the line, $y_p=\mathcal{B}/2$, in the direction of $\theta_p = 0$, where $y_p$ is the $y$-coordinate value and $\theta_p$ is the direction of motion on the pass. Consecutive passes in the boustrophedon path have opposite direction of motion and are $\mathcal{B}$ distance away from each other.

\input{baselines}

\input{snake_planner}
\input{jump_planner}
